CS-TRD: a Cross Sections Tree Ring Detection method

This work describes a Tree Ring Detection method for complete Cross-Sections of Trees (CS-TRD) that detects, processes and connects edges corresponding to the tree's growth rings. The method depends on the parameters for the Canny Devernay edge detector (sigma), a resize factor, the number of rays, and the pith location. The first five are fixed by default. The pith location can be marked manually or using an automatic pith detection algorithm. Besides the pith localization, CS-TRD is fully automated and achieves an F-Score of 89% in the UruDendro dataset (of Pinus taeda) and 97% in the Kennel dataset (of Abies alba) without specialized hardware requirements.

==> CSTRD_IPOL_v1/algos.tex <==
\Cref{algo:Globalalgo} depicts the CS-TRD method and \Cref{fig:algo} illustrates its intermediate results. The input is an image of a tree slice. First, we subtract the background, applying a deep learning-based approach \cite{salientObject} based on a two-level nested U-structure ($U^2Net$). %\Cref{fig:BackgroundExtraction} shows an example of such a procedure. 
Given the image without a background as shown in \Cref{fig:algo}.b, we must find the set of pixel chains representing the annual rings (dark to clear transitions). We need the center $c=(cy,cx)$ of the \textit{spider web} (the tree's pith) as input. This fundamental point can be manually marked or can be automatically detected \cite{ipolPith}. Here, we consider that this point is given (in the demo, both options are available).  Note that the values of parameters $\alpha$,  $N_{r}$, and $m_{c}$ are fixed once and for all.



\begin{figure*}
\begin{center}
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/F03d_with_background.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/F03d_segmentation.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/F03d_preprocessing.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/F03d_edges.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/F03d_filter.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/f03d_chains.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/f03d_connect.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/f03d_postprocessing.jpg}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/f03d_output.jpg}
   \caption{}
   \end{subfigure}   
      \caption{Principal steps of the CS-TRD algorithm: (a) Original image, (b) Background subtraction, (c) Pre-processed image (resized,  equalized, grayscale conversion), (d) Canny Devernay edge detector, (e) Edges filtered by the direction of the gradient, (f) Detected chains, (g) Connected chains, (h) Post-processed chains and (i) Detected tree-rings.}
   \label{fig:algo}
\end{center}
\end{figure*}


\begin{algorithm}[!htbp]
  \KwIn{$Im_{in}$, // segmented input image. Background pixels are set to 255 (white)  \\ 
        $cy$, $cx$, // pith's coordinates, in pixels: center of the \textit{spider web}  \\
        %$cx$, // pith's coordinate x, in pixels: center of the \textit{spider web} \\
        $\sigma$, // Canny edge detector gaussian kernel parameter \\
        %$th_{low}$, // low threshold on the module of the gradient. Canny edge detector parameter \\
        %$th_{high}$, // high threshold on the module of the gradient. Canny edge detector  parameter \\
        $height$, $width$, // dimensions of the image after the resize step \\
        %$width$, // width of the image after the resize step  \\
        $\alpha$, // threshold on the collinearity of the edge filtering \\
        $N_{r}$, // number of rays \\
        $m_{c}$ // minimum chain length \\
   }
  \KwOut{A json object $l\_rings$, each element is a closed \textit{chain} representing a tree-ring.}
  \SetAlgoLined
  \LinesNumbered
  \BlankLine 
    $Im_{pre}, cy, cx$ $\leftarrow$ preprocessing($Im_{in}, height, width, cy, cx$) \\
    $m\_ch_{e}, G_x, G_y$ $\leftarrow$ canny\_deverney\_edge\_detector($Im_{pre}$, $\sigma$) //  described in \cite{DevernayIPOL} \\
    $l\_ch_{f}$ $\leftarrow$ filter\_edges($m\_ch_{e}$,  $cy$, $cx$, $G_x$, $G_y$, $\alpha$, $Im_{pre}$)\\
    %$l\_ch_{f}$ $\leftarrow$ filter\_edges($m\_ch_{e}$,  $cy$, $cx$, $G_x$, $G_y$, $Im_{pre}$) //see \Cref{algo:ChainFilter} \\
    $l\_ch_{s},l\_nodes_s$ $\leftarrow$ sampling\_edges($l\_ch_{f}$, $cy$, $cx$, $N_r$, $m_c$, $Im_{pre}$)\\
    %$l\_ch_{s},l\_nodes_s$ $\leftarrow$ sampling\_edges($l\_ch_{f}$, $cy$, $cx$, $Im_{pre}$) //see \Cref{algo:samplingEdges} \\
    $l\_ch_{c},l\_nodes_c$ $\leftarrow$ connect\_chains($l\_ch_{s}$, $l\_nodes_s$, $cy$, $cx$) \\
    $l\_ch_p$ $\leftarrow$ postprocessing($l\_ch_{c}$, $l\_nodes_c$)\\
    $l\_rings$ $\leftarrow$ chain\_to\_labelme\_json($l\_ch_{p}$, $height$, $width$, $cy$, $cx$, $Im_{in}$) \\
    \KwRet{$l\_rings$}
\caption{Tree-ring detection algorithm}
\label{algo:Globalalgo}
\end{algorithm}

% \begin{figure}
%    \begin{center}
%    \begin{subfigure}{0.45\textwidth}
%    \includegraphics[width=1\textwidth]{figures/f02a_u2net_input}
%    \caption{}
%    \end{subfigure}
%    \hfill   
%    \begin{subfigure}{0.45\textwidth}
%    \includegraphics[width=1\textwidth]{figures/f02a_u2net_output}
%    \caption{}
%    \end{subfigure}
%    \caption{Background removal stage. Input (a) and output (b) using the code available from \cite{salientObject} } 
%    \label{fig:BackgroundExtraction}
% \end{center}
% \end{figure}

\subsection{Preprocessing} 
The first step in \Cref{algo:Globalalgo} is to preprocess the input image to increase the method's performance. We resize the image to a fixed $1500 \times 1500$ pixels size via Lanczos interpolation, then convert it to grayscale, and a histogram equalization is applied (\Cref{fig:algo}.c).

\subsection{Canny-Devernay edge detector} 
Line 2 of \Cref{algo:Globalalgo} corresponds to the edge detection stage. We apply the sub-pixel precision Canny Devernay edge detector \cite{Devernay95anon-maxima, DevernayIPOL}. The output of this step is a list of pixel chains corresponding to the image edges. Besides some noise-derived ones, we can group those edges into three  classes: 

\begin{itemize}
    \item $Edges_T$: produced by the tree growing process. It includes the edges that form the rings. Considering a pith outward direction, they can be of two types: those produced by early wood to late wood transitions (clear to dark) and latewood to early wood transitions (dark to clear). We are interested in detecting the former ones, hereon called annual rings.
    \item $Edges_R$: radial edges produced by cracks, fungi, or other phenomena.
    \item Other edges produced by wood knots and noise.
\end{itemize}

The gradient vector is normal to the edge and encodes the local direction and sense of the transition. The Canny Devernay filter produces the $G_x$ and $G_y$ matrices with  $x$ and $y$ gradient components, respectively, and $m\_ch_{e}$, the matrix of edge chains, in which successive rows list the coordinates $(x,y)$ of the chained pixels of a given edge, and the row [-1,-1] signals the end of an edge chain.

%The output,  $m\_ch_e$, is a matrix where each row refers to the edges' coordinates $(x,y)$. Each Devernay curve in the list is separated from the next one by a $(-1,-1)$.

%Despite the Canny Devernay edge detector having several parameters, we only adjust the standard deviation of the Gaussian kernel, $\sigma$. \Cref{exp:size} explain the procedure. Image output of this stage is shown in \Cref{fig:algo}.d.

The Canny Devernay edge detector has three parameters: The standard deviation of the Gaussian kernel $\sigma$, and the gradient modulus thresholds $th_{low}$ and $th_{high}$, associated with the threshold with hysteresis filtering on the edge points. We only adjust the parameter $\sigma$; the other two are fixed (see \Cref{exp:size}). \Cref{fig:algo}.d show the output of this stage. We slightly modify the Canny Devernay filter IPOL implementation \cite{DevernayIPOL} to get the matrices $G_x$ and $G_y$ as output. 


% \begin{itemize}
%     \item $\sigma$: The standard deviation of the Gaussian kernel. 
%      \item $th_{low}$ and $th_{high}$: Gradient threshold low and high, respectively, applied to the gradient modulus and associated with the two threshold hysteresis filtering on the edge points.
%\end{itemize}

%We build a Python wrapper to execute the IPOL Devernay-Canny implementation from \cite{DevernayIPOL} and feed the Devernay-Canny with the preprocessed image $Im_{pre}$ saved in disk in PGM format.


\subsection{Filtering the edge chains} 
Line 3 of  \Cref{algo:Globalalgo} corresponds to the edge filtering stage. Given the center $c=(cy,cx)$ and a point $p_i$ over an edge \textit{curve}, the angle $\delta(\vec{c p_i},\vec{G_{p_i}})$ between the vector $\vec{c p_i}$ %at the point  $p_i$  
and the gradient vector $\vec{G_{p_i}}$ at the the point  $p_i$  is given by:

 \begin{equation}
 \delta(\vec{c p_i},\vec{G_{p_i}}) =\arccos\left( \frac{\vec{c p_i} \times \vec{G_{p_i}}}{\|\vec{c p_i}\|\|\vec{G_{p_i}}\|}\right) \label{equ:filter_angle}   
 \end{equation}

We filter out all \textit{points} $p_i$ for which $
 \delta(\vec{c p_i},\vec{G_{p_i}})   \geq \alpha$. We fix  $\alpha = 30$ degrees. 
 
Two edge groups are filtered out: early wood transitions of the $Edges_T$ set gradients, which point inward, and $Edges_R$ set gradients, roughly normal to the \textit{rays}.  The algorithm produces the list $l\_ch_f$, including mainly the ring's edges and a disk border chain in the last position. \Cref{fig:algo}.e show the output of this stage.

% The filter edges method is shown at  \Cref{algo:ChainFilter}. It gets as input the Deverney edges $m\_ch_e$, the pith center, the image gradient components in the form of two matrices $G_x$ and $G_y$ and the preprocessed image $Im_{pre}$. As a parameter, it needs the threshold $\alpha$ of \Cref{equ:filter}. From lines 1 to  5, it computes the angle between vector $\vec{c p_i}$ and the gradient $\vec{G_{p_i}}$ at point $p_i$. We use the Python \textit{numpy} library matrix operations to speed up computation. 
% In line 1, we change the edges reference axis relative to the pith location, pixel ($c_y$, $c_x$). 
% %Figure \ref{fig:edge_filtering_change_reference} shows vectors $\Vec{O p_i}$ and $\Vec{c p_i}$, as well as the gradient $\vec{G_{p_i}}$ at edge point $p_i$. The function \textit{change\_reference\_axis} changes the vector coordinate reference from $\vec{O p_i}$ to $\vec{c p_i}$ and produces a new matrix $Xb$. This is made by subtracting the pith vector from each row. Matrix $Xb$ still has the delimiting edges curve rows with the value [-1,-1]

% Each edge gradient is saved in matrix $G$ (line 2), keeping the same edge order of the matrix $m\_ch_e$; this means that 
% \begin{equation*}
%    p_i = m\_ch_e[i] \rightarrow \vec{G_{p_i}} = G[i] 
% \end{equation*}
% Where $p_i$ is the i-row of matrix $m\_ch_e$ and $\vec{G_{p_i}}$ is the i-row of matrix $G[i]$.

% In Lines 3 and 4, the matrices $Xb.T$($Xb$ transposed matrix) and $G$ are normalized, dividing the vector by the norm as shown in  \Cref{equ:filter_angle_normalized},  simplifying \Cref{equ:filter_angle}:


% \begin{equation}
% \delta(R_i,\vec{G_{p_i}}) =\arccos\left( \frac{\vec{c p_i} \times \vec{G_{p_i}}}{\|\vec{c p_i}\|\|\vec{G_{p_i}}\|}\right) =  \arccos\left( \frac{\vec{c p_i}}{\|\vec{c p_i}\|} \times \frac{\vec{G_{p_i}}}{\|\vec{G_{p_i}}\|}\right)  = \arccos\left( \vec{c p_i}_{unit} \times \vec{G_{p_i}}_{unit}\right)  \label{equ:filter_angle_normalized}   
% \end{equation}

% In line 5, \Cref{equ:filter_angle_normalized} is computed in matrix form, and the angle between normalized vectors  $\vec{G_{p_i}}_{unit}$ and  $\vec{c p_i}_{unit}$ is returned in degrees in matrix $\theta$. In line 6, the edge filtering is applied, following  \Cref{equ: filter}. If the  edge point $p_i$ is filtered out, then  $X_{edges\_filtered}[i]=[-1,-1]$. The edges are converted to  \textbf{curve} objects in line 7. We say that two edge pixels belong to the same edge if,  between them, there does not exist a row in matrix $X_{edges\_filtered}$ with values [-1,-1]. The object \textbf{Curve} inherits the properties of the class \textbf{LineString} from the \textbf{Shapely} library\footnote{version 1.7} \cite{shapely}, which is used in the \textit{sampling edges} stage. Finally, in lines 8 and 9, the curve belonging to the border edges is computed and added to the curve list, $l\_ch_f$. In this context, the limits of the segmented image concerning the background are named $border$. 

% The function $get\_border\_curve$ is shown in \Cref{algo:get_border}. We use a simple method to compute the border edges. First, we generate a mask, an image of the same dimensions as $Im_{pre}$, enlarged by $3$ lines and $3$ columns before the first and after the last line and column to avoid border effects of the filtering. The mask image has two values: $0$ for the region of the wood slice and $255$ for the background. Lines 1 to 4  calculate the mask image. In line 1
% we threshold $Im_{pre}$ masking all the pixels with a value equal to 255, particularly the background. Some internal pixels can also have a value equal to 255. To avoid those pixels in the mask, we blur the mask (line 2), using a Gaussian Kernel with a high $\sigma$ (in our implementation $\sigma = 11$), and we set to 255 all the pixels with a value higher than 0 (lines 2 and 3). In line 4, the mask is padded with $pad = 3$.  Finally, in line 5, we apply an OpenCV finding contour method to get the border contour on the mask. The OpenCV implementation returns all the contours it finds, including the image's border. We select the contour for which the enclosed area is closest to half the image. This is a criterion that works fine for this purpose.  In line 6, the contour object is converted to a \textbf{Curve} object.

% \begin{algorithm}[!htbp]
%   \KwIn{$m\_ch_{e}$, // matrix of edge \textit{curves}  \\ 
%         $cy$, // pith's coordinate y, in pixels: center of the \textit{spider web}  \\
%         $cx$, // pith's coordinate x, in pixels: center of the \textit{spider web} \\
%         $G_x$, // X component of the gradient, a matrix\\
%         $G_y$, // Y component of the gradient, a matrix\\
%         $Im_{pre}$, // Preprocessed image\\
%         Parameter:\\
%         $\alpha$, //Threshold edge filter, \Cref{equ:filter}\\
%    }
%   \KwOut{A list $l\_ch^{k}_{f}$, $k=1,2, \cdots, N$, where each element is a filtered  edge \textit{curve}}
%   \SetAlgoLined
%   \LinesNumbered
%   \BlankLine 
%     $Xb$ $\leftarrow$  change\_reference\_axis($m\_ch_e$, $c_y$, $c_x$)// New origin is the pith center \\
%     $G$ $\leftarrow$  get\_gradient\_vector\_for\_each\_edge\_pixel($m\_ch_e$, $G_x$, $G_y$)\\
%     $Xb_{normalized}$ $\leftarrow$  normalized\_row\_matrix(Xb.T)\\
%     $G_{normalized}$ $\leftarrow$  normalized\_row\_matrix(G)\\
%     $\theta$ $\leftarrow$  compute\_angle\_between\_gradient\_and\_edges($Xb_{normalized}$, $G_{normalized}$)\\
%     $X_{edges\_filtered}$ $\leftarrow$  filter\_edges\_by\_threshold($m\_ch_e$, $\theta$, $\alpha$)\\
%     $l\_ch_f$ $\leftarrow$  convert\_masked\_pixels\_to\_curves($X_{edges\_filtered}$)\\
%     $border\_curve$ $\leftarrow$  get\_border\_curve($Im_{pre}$, $l\_ch_f$)// See  \Cref{algo:get_border}\\
%     $l\_ch_f$ $\leftarrow$  $l\_ch_f$ + $border\_curve$\\
%     \KwRet{$l\_ch_f$}
% \caption{filter\_edges}
% \label{algo:ChainFilter}
% \end{algorithm}

%\begin{figure}
%\begin{center}
%\def\svgwidth{0.35\linewidth}
%\input{edges_filtering.pdf_tex}
%\caption{Coordinates reference of edge $p_i$, vector $\Vec{O p_i}$. Edge filtering computation use vector $\Vec{c p_i}$. $O$ represents the origin of the image coordinate axis, $c$ represents the pith position and $\delta$ represents the angle between $\Vec{G_{pi}}$ and $\Vec{c p_i}$ ( \Cref{equ:filter_angle}).} 
%\label{fig:edge_filtering_change_reference}
%\end{center}
%\end{figure}


% \begin{figure}
% \begin{center}
%    \begin{subfigure}{0.35\textwidth}
%    \def\svgwidth{\linewidth}
%    \input{edges_filtering.pdf_tex}
%    \caption{} 
%    \label{fig:edge_filtering_change_reference}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}{0.35\textwidth}
%    \def\svgwidth{\linewidth}
%    \input{radii_angle.pdf_tex}
%    \caption{}.
%    \label{fig:radii_angle}
%    \end{subfigure}
%    \caption{(a) Coordinates reference of edge $p_i$, vector $\Vec{O p_i}$. The edge computation uses vector $\Vec{c p_i}$. $O$ represents the origin of the image coordinates, $c$ is the pith position and $\delta$ is the angle between the direction fo the gradient in $p_i$, $\Vec{G_{p_i}}$ and $\Vec{c p_i}$ (\Cref{equ:filter_angle}). (b) Ray references the axis. $C$ is the pith, $\theta_j$ is the angle associated to radii $r_j$}.
% \end{center}
% \end{figure}


% \begin{algorithm}[!htbp]
% \KwIn{$Im_{pre}$, // Preprocessed image \\
% $l\_ch_f$, //list of object Curves
% }
% \KwOut{$border\_curve$}
% \SetAlgoLined
% \LinesNumbered
% \BlankLine 
% $mask$ $\leftarrow$  mask\_background($Im_{pre}$)\\
% $mask$ $\leftarrow$  blur($mask$)\\
% $mask$ $\leftarrow$  thresholding($mask$)\\
% $mask$ $\leftarrow$  padding\_mask($mask$)\\
% $border\_contour$ $\leftarrow$  find\_border\_contour($mask$, $Im_{pre}$)\\
% $border\_curve$ $\leftarrow$  contour\_to\_curve($border\_contour$, len($l\_ch_f$))\\
% \KwRet{$border\_curve$}
% \caption{get\_border\_curve}
% \label{algo:get_border}
% \end{algorithm}

\subsection{Sampling edges} Line 4 of  \Cref{algo:Globalalgo}, is the edge sampling stage which produces the \textit{nodes} depicted in \Cref{fig:definitions}.b. We sample each \textit{curve} of the $l\_ch_{f}$ list using the number of rays  $N_r$. The algorithm has two parameters: $N_r$ (360 by default) and $m_c$, the minimum number of nodes in a \textit{chain}. Every \textit{chain} has two endpoints, so we fix  $m_c=2$. The algorithm produces two lists: $l\_ch_{s}$ (of \textbf{Chain} objects)  and  $l\_nodes_{s}$ (of \textbf{Nodes} objects), which includes the nodes of all chains. These lists include two artificial \textit{chains}, one of type \textit{center} with $N_r$ nodes with the exact pith coordinates but different angular orientations, and one corresponding to the border. %\Cref{algo:get_border} illustrates how the border Devernay curve is computed. 
The inclusion of these artificial chains is beneficial for the connecting chain stage. The attribute $type$ of the object \textbf{Chain} identifies if it is an artificial or a standard chain.  

\Cref{fig:algo}.f shows this stage output. Standard chains are in red, and center and border chains are in black. Due to the sampling, there are fewer chains than edges. \Cref{fig:algo}.e has more (noisy) curves around the pith than \Cref{fig:algo}.f. Some small curves whose sampled length is shorter than $m_{c}$ are discarded. In that sense, this parameter filters out "short" chains.

%The object \textbf{Chain} contains a list of pointers to all the nodes belonging to that \textit{chain} ($l\_nodes$). This allows us to find the nodes of a given \textit{chain}. The object \textbf{Node} contains the identifier of the \textit{chain} to which it belongs ($chain\_id$). There is no \textit{chain} without nodes, nor nodes belonging to more than one \textit{chain}.

% An object \textbf{Chain} has the following attributes:
% \begin{itemize}
%     \item $l\_nodes$: a chained list of the nodes belonging to the chain.
%     \item $id$: chain identification.
%     \item $N_r$: total number of rays on the disk.
%     \item $extA$: first endpoint of the chain, named node A.
%     \item $extB$: second endpoint of the chain, named node B.
%     \item $type$: We define three chain types: border, normal, and center.
%     \item $B\_outward$: Pointer to the next chain above the B node.
%     \item $B\_inward$: Pointer to the next chain below the B node.
%     \item $A\_outward$: Pointer to the next chain above the A node.
%     \item $A\_inward$: Pointer to the next chain below the A node.
%\end{itemize}

Every chain has two endpoint nodes, A and B. Endpoint A is always the furthest node clockwise, while endpoint B is the most distant node counterclockwise. We use the concepts of \textit{outward} and \textit{inward} (concerning a given endpoint) in the chain attributes. Given the corresponding \textit{ray} of a \textit{chain} endpoint, we find the first \textit{chain} that intersects it going from the chain to the center along the \textit{ray} (named \textit{inward}) and the first \textit{chain} that intersects that \textit{ray} moving away from the center (named \textit{outward}), as shown in \Cref{fig:cproperties}. Chains are superposed over the gray-level image. The ray at endpoint A is blue, and the nodes are red and lie at the intersection between the rays and the edges. Orange and yellow chains are the \textit{visible} ones for the black chain at endpoint A (outward and inward, respectively). 

% An Object \textbf{Node}  has the following attributes:
% \begin{itemize}
%     \item $(x,y)$ node coordinates. Floating point numbers.
%     \item $chain\_id$: identification of the chain to which the node belongs.
%     \item $radial\_distance$: Euclidean distance to the center. It is a floating point number.
%     \item $angle$: angle orientation of the ray passing by that node, in degrees. It is a floating point number.
% \end{itemize}

We use three metric distances between chains. Given $EndPoint_{j}$ for the current chain $Ch_j$, and  $EndPoint_{k}$ for chain $Ch_k$, distances are defined as:

\begin{itemize}
\item \textbf{ Euclidean } defined as 
\begin{equation}
d_e = \sqrt{\left(x_j-x_k\right)^{2} + \left(y_j-y_k\right)^{2}}   \label{equ: Euclidean}
\end{equation}
Where $(x_j, y_j)$ and $(x_k, y_k)$ are the cartesian coordinates of $EndPoint_j$ and $EndPoint_k$.

\item \textbf{Radial Difference} defined as 
\begin{equation}
d_{rd} = \|r_j - r_k\|    \label{equ:radial}
\end{equation}
$r_j$ is the  Euclidean distance between $EndPoint_j$ and the pith center, and $r_k$ is the  Euclidean distance between $EndPoint_k$ and the pith center.

\item \textbf{Angular} Given the endpoints ray support angle, $\theta_j$ and $\theta_k$, this distance is defined as 
\begin{equation}
d_a =    \left(\theta_j-\theta_k+360\right) mod \hspace{0.2cm} 360 \label{equ:angular}
\end{equation}
Where $\theta_j$ and $\theta_k$ are the ray's direction supporting $EndPoint_j$ and $EndPoint_k$ (both in degrees), respectively, and $mod$ refers to the module operation.  %\Cref{fig:radii_angle} illustrates angle $\theta_j$ of $r_j$  given the disk pith position $c$.
\end{itemize}

%\begin{figure}
%\begin{center}
%   \def\svgwidth{0.3\linewidth}
%   \input{radii_angle.pdf_tex}
%    \caption{ Ray references axis. $C$ is the pith center. $\theta_j$ is the angle of radii $r_j$}.
%   \label{fig:radii_angle}
%\end{center}
%\end{figure}


%\Cref{algo:samplingEdges} extract the image dimensions from the  preprocessed image   $Im_{pre}$. Then, we proceed to build the rays. A ray object is a semi-line, with one endpoint at the center $c=(cy,cx)$ (the pith) and the other at the image border. This gives a list of $N_r$ rays. Then, at line 3,  we compute the intersections between \textit{curves} and rays using the \textbf{Shapely} python library.
%Note that a \textit{curve} produced by Devernay is a set of chained pixels some of which are also nodes, as shown in Figure \ref{fig:definitionsB}. Once the Nodes are found, we create a \textit{chain} including only the nodes and not all the points of the corresponding Devernay \textit{curve}. In this sense, a \textit{chain} is a sampled \textit{curve}. If a \textit{chain} has less than \textbf{$min\_chain\_length$} nodes, we delete it. 


\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{chain_properties.png}
    \caption{A given chain (in black) with two endpoints A and B. Its nodes (in red) appear at the intersection between the Canny Devernay curve and the rays. The ray at endpoint A is in blue. Other chains detected by Canny Devernay are in white. Endpoint A's inward and outward chains are in yellow and orange, respectively.}
    \label{fig:cproperties}
\end{figure}

% \begin{algorithm}[!htbp]
%   \KwIn{
%   $l\_ch_{f}$, // list of \textit{curves} \\ 
%   $cy$, // pith's coordinate y, in pixels: center of the \textit{spider web}  \\
%   $cx$, // pith's coordinate x, in pixels: center of the \textit{spider web} \\
%   $Im_{pre}$ // preprocessed image  \\
%   Parameters: \\
% $min\_chain\_length$, //  minimum length of a chain \\
% $N_r$ // number of total rays\\
%   }
%   \KwOut{A list $l\_ch^{k}_{s}$, $k=1,2, \cdots, N$, where each element is a \textit{chain}; \\
%   $l\_nodes^{k}_{s}$, $k=1,2, \cdots, N_n$, where each element is a \textit{Node}\\}
%   \SetAlgoLined
%   \LinesNumbered
%   \BlankLine 
% $height$, $width$ $\leftarrow$ $Im_{pre}$.shape\\
% $l\_rays$ $\leftarrow$ build\_rays($N_r$, $height$, $width$, $cy$, $cx$)\\
%  $l\_ch_{s}$,$l\_nodes_s$ $\leftarrow$ intersections\_between\_rays\_and\_devernay\_curves($cy$, $cx$, $l\_rays$ , $l\_ch_f$, $min\_chain\_length$, $N_r$, $height$, $width$) \\
% \tcc{Virtual center chain is added in the input list $l\_ch_s$. Additionally, its nodes are added in  $l\_nodes_s$}
% generate\_virtual\_center\_chain($cy$, $cx$, nr, $l\_ch_s$,  $l\_nodes_s$, $height$, $width$)\\
%    \KwRet{$l\_ch_{s}$,$l\_nodes_s$}
% \caption{sampling\_edges}
% \label{algo:samplingEdges}
% \end{algorithm}


\subsection{Connect chains}
\label{connect} 
We must now group these chains to form the rings (Line 5 of  \Cref{algo:Globalalgo}). As this section is one of the main parts of the algorithm, we will divide it into two subsections: one that explains the general idea of chain connection and another that details the algorithms themselves.

\subsubsection{General Logic of Chain Connection}
\label{sec:connect_general_logic}

The input of the algorithm is a set of chains. Some of these chains are spurious, produced by noise, small cracks, knots, etc., but most are part of the desired rings, as seen in Figure \ref{fig:algo}.f.

In general, several chains form a ring. To connect them, we must decide if the endpoints of two given chains can be connected, as illustrated by \Cref{fig:connectivityIssue}.a. We use a support chain ($Ch_0$ in the figure) to determine if those chains must be connected.

\begin{figure}
\begin{center}
   \begin{subfigure}{0.45\textwidth}
    \def\svgwidth{\linewidth}
    \input{ChainYtresChainsYnodos.pdf_tex}
    \caption{} 
    \end{subfigure}
    %\hfill
   \begin{subfigure}{0.45\textwidth}
    \def\svgwidth{\linewidth}\input{ChainYtresChainsYnodosIntersectados.pdf_tex}
    \caption{} 
    \end{subfigure}
    \caption{An illustration of the \textit{connectivity} issue. (a) The question is if endpoint \textit{A} of $Ch_3$ must be connected to endpoint \textit{B} of $Ch_2$ (red dashed line) or to endpoint \textit{B} of $Ch_1$ (blue dashed line). In figure (b), the same question can be posed for the connection between endpoint B of $Ch_1$ and endpoint A of $Ch_2$. This connection is forbidden because $Ch_1$ and $Ch_2$ intersect (the endpoints are on the same \textit{ray}). Note that we represent the connections by line segments for clarity, but these are curves in the image space, as we interpolate between \textit{chain} endpoints in polar geometry.} 
   \label{fig:connectivityIssue}
\end{center}
\end{figure}


\begin{figure}[ht]
\begin{center}
   \begin{subfigure}{0.47\textwidth}
   \def\svgwidth{\linewidth}
   \input{CincoChains.pdf_tex}
    \caption{}
%   \label{fig:candidatas}
   \end{subfigure}
   \begin{subfigure}{0.47\textwidth}
   \def\svgwidth{\linewidth}
   \input{ConnectivityMeasuresV1.pdf_tex}
    \caption{}
%   \label{fig:connectivity}
   \end{subfigure}
\begin{subfigure}{0.47\textwidth}
   \def\svgwidth{\linewidth}
   \input{derivative_goodness.pdf_tex}
    \caption{}
%   \label{fig:derivative_goodness}
\end{subfigure}
\caption{Connectivity nomenclature. (a) For the \textit{chain support} $Ch_0$, the set of  \textit{chain candidates} is formed by $Ch_1$, $Ch_2$, $Ch_4$, $Ch_5$ and $Ch_6$. \textit{Chain} $Ch_3$ is shadowed  by $Ch_1$ but $Ch_5$ is not shadowed by  $Ch_6$ because at least one endpoint of $Ch_5$ is visible from $Ch_0$. Note that a \textit{chain} becomes part of the \textit{candidate chains set} if at least one of its endpoints is visible from the \textit{chain support}. (b) Quantities used to measure the connectivity between \textit{chains}. $\delta R_i$ is the radial difference between two successive \textit{chains} along a \textit{ray} $R_i$ and $\delta N_i$ is the radial difference between two successive \textit{nodes} $N_i$ and $N_{i+1}$. Note that these nodes can be part of the same \textit{chain} or be part of two different \textit{chains} that may be merged. $Ch_i$ is the support chain. $Ch_i$ visible chains are $Ch_j$, $Ch_l$ and $Ch_k$. Chains $Ch_j$ and $Ch_k$ satisfy similarity conditions. (c) Chains $Ch_j$ and $Ch_k$ are candidates to be connected, and  $Ch_{i}$ is the support chain. $N_j^n$ ($N_k^n$) are the nodes of $Ch_j$ ($Ch_k$), with $n=0$ for the endpoint to be connected, and $r_s$ represents the radial distance to the center of $Node^s$. In red are the nodes created by an interpolation process between both endpoints.}.
\label{fig:ConnectivityNomenclature}
\end{center}
\end{figure}

To group chains that belong to the same ring, we proceed as follows:
\begin{enumerate}
    \item We order all the chains by length and begin by processing the longest, which we call \textit{Chain support}, $Ch_i$. Once we finish merging all the possible \textit{candidate chains} related to that one (the set $candidates_{Ch_i}$), we do the same with the next longest \textit{chain}, and so on. The reason for processing the longest chains first is that longer chains contain more edge information and more information about the tree ring structure, giving more robust results. % The logic behind this is that 
    Longer chains are more likely to be an edge belonging to an annual tree ring. Since consecutive rings have similar shapes, this iteration method propagates the shape of the longer chains.

        \item We find the chains that are visible from the \textit{Chain support} inwards (i.e., in the direction from \textit{Chain support} to the center). %The concept of \textit{visibility} here means that at least one endpoint of the \textit{candidate chain} is visible from the \textit{Chain support}. 
    Here, \textit{visible} means that a \textit{ray} that goes through one \textit{candidate chain} endpoint crosses the \textit{chain support} without crossing any other \textit{chains} in between. The set of \textit{candidate chains} of the \textit{Chain support} $Ch_i$ is named \textit{$candidates_{Ch_i}$}.  In \Cref{fig:ConnectivityNomenclature}.a this set is $candidates_{Ch_0} = \{Ch_1, Ch_2, Ch_4, Ch_5, Ch_6\} $.
    \textit{Chain} $Ch_3$ is shadowed  by $Ch_1$ and $Ch_5$ is not shadowed by $Ch_6$ because at least one of its endpoints are visible from $Ch_0$. The same process is made for the chains visible from the \textit{Chain support} outwards.

    \item We explore the set \textit{$candidates_{Ch_i}$} searching for  connections between them. By construction, the \textit{chain support} is not a candidate to be merged in this step. From the endpoint of a chain, we move forward angularly. The next endpoint of a nonintersecting \textit{chain} in \textit{$candidates_{Ch_i}$}  is a candidate to be connected to the first one. We say that two \textit{chains} intersect if there exists at least one \textit{ray} that crosses both \textit{chains}. For example, in Figure \ref{fig:ConnectivityNomenclature}.a, $Ch_6$  intersects with $Ch_5$ but not with $Ch_4$. 
    \label{connect:item_recorrer_cadenas}
    \item \label{connect:item_connectiviy_goodness} To decide if both chains must be connected, we must measure the \textit{connectivity goodness} between them, combining four criteria:
    \begin{enumerate}
        \item \textit{Radial tolerance for connecting chains}. The radial difference between the distance from each chain to be merged (measured at the endpoint to be connected) and the support chain must be small. For example, in Figure \ref{fig:ConnectivityNomenclature}.b, if we want to connect node $N_i$ of $Ch_l$ and node $N_{i+1}$ of $Ch_k$, we must  verify that $$ \delta R_i*(1-Th_{Radial\_tolerance})\leq \delta R_{i+1} \leq \delta R_i*(1+Th_{Radial\_tolerance})$$ Where $Th_{Radial\_tolerance}$ is a parameter of the algorithm. We call this condition \textit{RadialTol}. 

    
%\begin{figure}
%\begin{center}
%   \def\svgwidth{0.45\linewidth}
%   \input{ConnectivityMeasuresV1.pdf_tex}
%    \caption{Quantities used to measure the connectivity between \textit{chains}. $\delta R_i$ is the radial difference between two successive \textit{chains} along a \textit{ray} $R_i$ and $\delta N_i$ is the radial difference between two successive \textit{nodes} $N_i$ and $N_{i+1}$. Note that these nodes can be part of the same \textit{chain} or be part of two different \textit{chains} that may be merged. Support chains are represented with the name $Ch_i$. $Ch_i$ visible chains are $Ch_j$, $Ch_l$ and $Ch_k$. Chains $Ch_j$ and $Ch_k$ satisfy similarity conditions}.
%   \label{fig:connectivity}
%\end{center}
%\end{figure}



        \item \textit{Similar radial distances of nodes in both chains}. For each chain, we define a set of nodes. For the chain $Ch_j$, this set is $N_j = \{ N_j^0, N_j^1,..., N_j^{n_{nodes}}\}$ where $n_{nodes}$ is the number of nodes to be considered,  fixed to $n_{nodes}=20$. See Figure \ref{fig:ConnectivityNomenclature}.c. We use the whole chain if it is shorter than $n_{nodes}$. We measure $\delta R_i$, the radial distance between each node in the given chain and the corresponding node (same ray) in the support chain, as illustrated in Figure \ref{fig:ConnectivityNomenclature}.b. This defines a set for each considered chain $j$ and $k$:
        $Set_j = \{ \delta R_j^0,..,\delta R_j^{n_{nodes}}\}$ and  $Set_k = \{ \delta R_k^0,..,\delta R_k^{n_{nodes}}\}$. We calculate its mean  and standard deviation $Set_j(\mu_j,\sigma_j)$ and $Set_k(\mu_k,\sigma_k)$. %\textit{$Th_{Distribution\_size}$}, an integer parameter, defines the distribution size. 
        This defines a range of radial distances associated with each chain: $Range_j = (\mu_j -    \textit{$Th_{Distribution\_size}$}*\sigma_j, \mu_j +  \textit{$Th_{Distribution\_size}$}*\sigma_j )$ and $Range_k = (\mu_k -   \textit{$Th_{Distribution\_size}$}*\sigma_k, \mu_k +   \textit{$Th_{Distribution\_size}$}*\sigma_k )$, where \textit{$Th_{Distribution\_size}$} is a parameter. There must be a non-null intersection between both distributions to connect both chains: $Range_j \cap Range_k \neq 0$. We call this condition \textit{SimilarRadialDist}.
        
        \item \textit{Regularity of the derivative}. Given two chains $Ch_j$ and $Ch_k$ which can be connected, let's call $Ch_{jk}$ the set of interpolated nodes between them (\Cref{fig:ConnectivityNomenclature}.c). The new virtual chain created by the connection between $Ch_j$ and $Ch_k$ will encompass the nodes of those two chains and $Ch_{jk}$. The parameter \textit{derivFromCenter} controls how are estimated the interpolated nodes between two chains, as the ones in red in   \Cref{fig:ConnectivityNomenclature}.c. If $derivFromCenter=1$, ray angle and radial distance from the center are used to estimate the position of the interpolated nodes. If its value is 0, the estimation is made by measuring the radial distance to the support chain. To test the regularity of the derivative, we define a set of nodes for each concerned chain. For the chain $Ch_j$, this set is $\{ N_j^0, N_j^1,..., N_j^{n_{nodes}}\}$ where $n_{nodes} = 20$ is the number of nodes to be considered. If the chain is shorter, we use all nodes. We compute the centered derivative in each node for all chains,  $\delta N^s = \frac{\|r_{s+1} - r_{s-1}\|}{2}$, where $r_s$ is the radial distance of the node $N^s$ to the center (i.e., the Euclidean distance between the node and the center). The set of the existing chains nodes is $Der(Ch_j, Ch_k) = \{\delta N_j^0, ..., \delta N_j^{n_{nodes}}, \delta N_k^0, ..., \delta N_k^{n_{nodes}} \} $. The condition \textit{RegularDeriv} is asserted if the greatest derivative in the interpolated chain is less or equal to the greater  derivative in the neighboring chains, with  tolerance $Th_{Regular\_derivative}$: 
        $$
        max(Der(Ch_{jk})) \leq max ( Der(Ch_j,Ch_k) ) \times Th_{Regular\_derivative} 
        $$

        \item \textit{Non-Overlapping Chain}. Finally, no other chain must exist between the chains to be connected. If another chain exists in between, it must be connected to the closer one. For example, in Figure \ref{fig:ConnectivityNomenclature}.a, it is impossible to connect chains $Ch_3$ and $Ch_5$ because between them appear $Ch_4$. We call this condition \textit{ExistChainOverlapping}. 
    \end{enumerate}
    Summarizing, in order to connect chains $Ch_j$ and $Ch_k$, the following condition must be met:
    
    \begin{equation}
            \mathbf{not}\textit{ExistChainOverlapping} \land \textit{RegularDeriv} \land ( \textit{SimilarRadialDist} \lor \textit{RadialTol} ) 
            \label{equ:similiraty_criterio}
    \end{equation}
    
    where $\lor$ and $\land$ stands for the logical \textit{or} and \textit{and} symbols, respectively, and the symbol $\mathbf{not}$ stands for the \textit{not} operator.
    
    The method iterates, searching for connectivity between chains over different neighborhood sizes. The parameter \textit{NeighbourdhoodSize} defines the maximum allowed distance, measured in degrees, for connecting two chains. %If the distance between the two chain endpoints is longer than \textit{NeighbourdhoodSize}, those chains are disconnected. 


    We iterate this process for the whole image nine times. In the first iteration, there are a lot of small chains, but in the second and third iterations, the concerned chains are already more extended and less noisy. As the merging process advances, we can relax the parameters to connect more robust chains. Table \ref{tab:connectivityParameters} summarizes the parameters used in each iteration. 


    \begin{table}[!htbp]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
    \hline
                       & 1   & 2   & 3   & 4   & 5   & 6   & 7   & 8   & 9   \\ \hline
    \textit{$Th_{Radial\_tolerance}$}        & 0.1 & 0.2 & 0.1 & 0.2 & 0.1 & 0.2 & 0.1 & 0.2 & 0.2 \\ \hline
    \textit{$Th_{Distribution\_size}$} & 2   & 2   & 3   & 3   & 3   & 3   & 2   & 3   & 3   \\ \hline
    \textit{$Th_{Regular\_derivative}$}      & 1.5 & 1.5 & 1.5 & 1.5 & 1.5 & 1.5 & 2   & 2   & 2   \\ \hline
    \textit{NeighbourdhoodSize} & 10  & 10  & 22  & 22  & 45  & 45  & 22  & 45  & 45  \\ \hline
    \textit{derivFromCenter }   & 0   & 0   & 0   & 0   & 0   & 0   & 1   & 1   & 1   \\ \hline
    \end{tabular}
    \caption{Connectivity Parameters. Each column is the parameter set used on that iteration.}
    \label{tab:connectivityParameters}
    \end{table}
        
        

    \item We proceed in the same manner in the outward direction.
\end{enumerate}


\subsubsection{Detailed Description of the Algorithms}

\Cref{algo:connectmainlogic} depicts the chain connection step's logic, described in the former section. %This algorithm takes as parameters the good connectivity conditions defined in \Cref{tab:connectivityParameters} ($th\_radial\_tolerance$, $th\_distribution\_size$, $th\_regular\_derivative$, $neighbourhood\_size$, $derivative\_from\_center$), where each column of the table defines a set of conditions. \Cref{algo:connectmainlogic} 
It is iteratively called from an external function (Line 5 of \Cref{algo:Globalalgo}) with the parameter values defined in  \Cref{tab:connectivityParameters} columns. Chains produced at one iteration become the input chains for the next one.

As was mentioned, the logic for connecting chains is based on iterating over the \textit{support chain}. For each one, the set of visible chains is selected. The logic for selecting the support chain in each iteration (line 1~\Cref{algo:connectmainlogic}) is encapsulated in the \textbf{SystemStatus} object, which is the hub of our \textit{system}, containing all the necessary information to operate. The \textit{system} comprises all the chains and nodes and the intersection matrix $M$. This binary square matrix stores the intersection information of chains at each iteration. Rows and columns of $M$ span the chain list. Chain $Ch_j$ intersect chain $Ch_k$ if $M[j,k] = 1$. We say that two chains intersect if at least one ray crosses both chains. The intersection matrix, $M$, is an input argument for \Cref{algo:connectmainlogic}. The \textbf{SystemStatus} object updates the chains and nodes lists and the matrix $M$ whenever two chains are connected. This update is critical for our operation and signifies that the \textit{system} has been modified.

\Cref{algo:connectmainlogic} has a main loop from lines 2 to 19. The \textbf{SystemStatus} object produces the support chain ($Ch_i$) in each iteration. To speed up the process, support chains are iterated by following a neighborhood logic instead of sequentially going over the list.  Given a support chain, a secondary loop (lines 5 to 18) iterates over the inward (or outward) visible chains, as described in \Cref{fig:ConnectivityNomenclature}.a. In a third inner loop (lines 11 to 18), each candidate chain ($Ch_j$) is examined to find the closest chain ($Ch_k$) that meets the similarity goodness criteria (\Cref{equ:similiraty_criterio}). In summary, we search for the nearest chains to endpoints \textit{$Ch_{k}^a$} and \textit{$Ch_{k}^b$}. Between these candidate chains, we select the closest one ($Ch_k$) that does not intersect with the original chain $Ch_j$. Then, in line 17, chains $Ch_j$ and $Ch_k$ are connected. Connecting two chains implies generating new nodes between them (the new chain cannot have "holes"). Once no more chains can be connected, the main loop (lines 2 to 19) exits. In line 20, we iterate over all the chains in $l\_ch_s$, and if one has enough nodes, we complete it. The output is the lists of chains ($l\_ch_c$), nodes ($l\_nodes_c$), and the intersection matrix, $M$.

\begin{algorithm}[!htbp]
\KwIn{
$l\_ch_{s}$, // chains list \\
$l\_nodes_s$, // nodes list \\
$M$, //Binary Matrix  with intersection chains info \\
$cy$, $cx$, // pith's coordinates, in pixels: center of the \textit{spider web}  \\
$N_r$, // total number of rays\\
Parameters: \\
$th\_radial\_tolerance$, // Radial tolerance for connecting chains \\
$th\_distribution\_size$, // Chains Radial Difference Standard deviations for connecting chains \\
$th\_regular\_derivative$, // Chains Radial Derivative threshold for connecting chains \\
$neighbourhood\_size$, //Maximum angular distance allowed for connecting chains \\
$derivative\_from\_center$ // Define how nodes are interpolated \\
}
\KwOut{A list $l\_ch_{c}$, where each element is  a \textit{chain}, \\
$l\_nodes_{c}$,  where each element is a \textit{Node},\\
$M$, intersection matrix updated}
%$State_{i-1}$ $\leftarrow$  0\\ 
%$State_{i}$ $\leftarrow$ init\_system($l\_ch_{s}$, $l\_nodes_s$, $M$ , $cy$, $cx$, $N_r$,$th\_radial\_tolerance$, $th\_distribution\_size$, $th\_regular\_derivative$, $neighbourhood\_size$, $derivative\_from\_center$)\\
$state$ $\leftarrow$  $SystemStatus$($l\_ch_{s}$, $l\_nodes_s$, $M$ , $cy$, $cx$, $N_r$,$th\_radial\_tolerance$, $th\_distribution\_size$, $th\_regular\_derivative$, $neighbourhood\_size$, $derivative\_from\_center$)\\
%\While{$State_{i} \neq State_{i-1}$}{
\While{$state$.continue\_in\_loop()}{
    $Ch_i$ $\leftarrow$ $state$.get\_next\_chain() %//See  \Cref{algo:get_next_chain}
    \\
    $l\_s\_outward$, $l\_s\_inward$ $\leftarrow$ get\_chains\_in\_and\_out\_wards($l\_ch_{s}$,$Ch_i$)\\
    \For{$l\_candidates\_{Ch_i}$ in ($l\_s\_outward$, $l\_s\_inward$)}{
        $j\_pointer$ $\leftarrow$ 0\\
        \If{$l\_candidates\_{Ch_i}$ =  $l\_s\_inward$}{
             $location$ $\leftarrow$ "inward"
        }
        \Else{
             $location$ $\leftarrow$ "outward"
        }

        \While{length($l\_candidates\_{Ch_i}$) $>$ $j\_pointer$}{
             $Ch_j$ $\leftarrow$ $l\_candidates\_{Ch_i}$[$j\_pointer$]\\
             $l\_no\_intersection\_j$ $\leftarrow$ get\_non\_intersection\_chains($M$, $l\_candidates\_{Ch_i}$, $Ch_j$)\\
             $Ch_k^b$ $\leftarrow$ get\_closest\_chain\_logic($state$, $l\_candidates\_{Ch_i}$, $Ch_j, l\_no\_intersection\_j, Ch_i, location$, $B$)\\%//See  \Cref{algo:get_closest_chain_logic}\\
             $Ch_k^a$ $\leftarrow$ get\_closest\_chain\_logic($state$, $l\_candidates\_{Ch_i}$, $Ch_j, l\_no\_intersection\_j, Ch_i, location$, $A$)\\%//See  \Cref{algo:get_closest_chain_logic}\\
             $Ch_k$, $endpoint$ $\leftarrow$ select\_closest\_one($Ch_j$, $Ch_k^a$, $Ch_k^b$)\\
             connect\_two\_chains($state$, $Ch_j$, $Ch_k$, $l\_candidates\_{Ch_i}$, $endpoint$, $Ch_i$)\\%//See  \Cref{algo:connect_two_chains}\\
             $j\_pointer$ $\leftarrow$ update\_pointer($Ch_j$, $Ch_k$, $l\_candidates\_{Ch_i}$)\\
        }
    }
    $state$.update\_system\_status( $Ch_i$, $l\_s\_outward$, $l\_s\_inward$)\\%//See  \Cref{algo:update_system}\\
}
$l\_ch_{c}$,$l\_nodes_{c}$, $M$ $\leftarrow$ iterate\_over\_chains\_list\_and\_complete\_them\_if\_met\_conditions($state$)\\

\SetAlgoLined
\LinesNumbered
\BlankLine 
\KwRet{$l\_ch_{c}$,$l\_nodes_{c}$, $M$}
\caption{Connect Chains Main Logic}
\label{algo:connectmainlogic}
\end{algorithm}

Once we have a support chain ($Ch_i$), we iterate over the visible chains to connect them if they meet the similarity criteria as briefly shown in \Cref{algo:connectmainlogic}. %The main pending algorithms are the selection of the closest chain given $Ch_j$ within the visibility set (\Cref{algo:get_closest_chain})  and the goodness conditions between two chains checking (\Cref{algo:connectivity_goodness_condition}). 

The method $get\_closest\_chain\_logic$ (lines 14 and 15 of \Cref{algo:connectmainlogic}) provides the closest chain,  performing a dual symmetry check: if chain $Ch_k$ is the closest to $Ch_j$, then the closest one to $Ch_k$ should also be $Ch_j$. %\Cref{algo:get_closest_chain}, invoked within the $get\_closest\_chain\_logic$ method implements the logic to find the closest chain to $Ch_j$. 
\Cref{algo:get_closest_chain} (function $get\_closest\_chain$), invoked within $get\_closest\_chain\_logic$, search for the closest candidate chain (described in \Cref{sec:connect_general_logic} item \ref{connect:item_recorrer_cadenas}) that meet conditions described in \Cref{sec:connect_general_logic} item \ref{connect:item_connectiviy_goodness}. In line 2, all chains in the neighborhood (defined by the $Ch_j$ endpoint and the $neighbourhood\_size$ $state$ attribute) are selected. For example, given the endpoint A with an angle of 0 degrees and $neighbourhood\_size=20$, all the chains included in $l\_candidates\_Ch_i$ with endpoint B angle in $[0-20,0]=[340,360]$ are selected and returned in ascending angular order concerning the endpoint of $Ch_j$. Lines 5 to 13 define the main loop. Two conditions determine an exit from the loop: either it exists a chain that satisfies conditions from \Cref{equ:similiraty_criterio} or no chains in the set $l\_sorted\_chains\_in\_neighbourhood$ satisfy the conditions. Line 7 of function \textbf{$connectivity\_goodness\_condition$} implements \Cref{equ:similiraty_criterio}. 

\begin{algorithm}[!htbp]
  \KwIn{$state$,\\
  $Ch_j$, // current chain   \\
  $l\_no\_intersection\_j$, // chains  that no intersect with $Ch_j$, set of candidates  to connect with $Ch_j$\\
  $Ch_i$, // support chain\\
  $location$, // inward o outward position of $Ch_j$ regarding to the support chain\\
  $endpoint$, // $Ch_j$ endpoint \\
  $M$, // intersection matrix\\
  }
\KwOut{closest chain to $Ch_j$ that satisfies the connectivity goodness conditions.\\}
\SetAlgoLined
\LinesNumbered
\BlankLine 
$neighbourhood\_size$ $\leftarrow$ $state.neighbourhood\_size$\\
$l\_sorted\_chains\_in\_neighbourhood$ $\leftarrow$ get\_chains\_in\_neighbourhood($neighbourhood\_size$, $l\_no\_intersection\_j$, $Ch_j$, $Ch_i$, $endpoint$, $location$)\\
$next\_id$ $\leftarrow$ 0\\
$Ch_k$ $\leftarrow$ None\\
\While{$len(l\_sorted\_chains\_in\_neighbourhood) > next\_id$}{
    $candidate\_chain$ $\leftarrow$ l\_sorted\_chains\_in\_neighbourhood[$next\_id$]\\
    $pass\_control$, $radial\_distance$ $\leftarrow$ connectivity\_goodness\_condition($state$, $Ch_j$, $candidate\_chain$, $Ch_i$, $endpoint$) // See  \Cref{algo:connectivity_goodness_condition}\\
    \If{$pass\_control$}{
        $Ch_k$ $\leftarrow$ get\_the\_closest\_chain\_by\_radial\_distance\_that\_does\_not\_intersect($Ch_j$, $endpoint$, $location$, $radial\_distance$, $candidate\_chain$, $M$, $l\_sorted\_chains\_neighbourhood$) // See Figure \ref{fig:connectivityIssue}.a \\%and  \Cref{algo:get_the_closest_chain_by_radial_distance_that_does_not_intersect}\\
        break\\
    }
    $next\_id$ $\leftarrow$ $next\_id$ + 1\\
}

\KwRet{$Ch_k$}
\caption{Get closest chain}
\label{algo:get_closest_chain}
\end{algorithm} 


\begin{figure}
\begin{center}
   \begin{subfigure}{0.47\textwidth}
    \def\svgwidth{\linewidth}
    \input{closest_chain.pdf_tex}
    \caption{} 
   %\label{fig:closest_chain} 
    \end{subfigure}
    %\vspace{5pt}
  %  \hfill
    \begin{subfigure}{0.30\textwidth}
    \def\svgwidth{\linewidth}
    \input{endpoints_condition.pdf_tex}
    \caption{}
   % \label{fig:endpoint_condition}
    \end{subfigure}
    \caption{Chains connection. (a) $Ch_i$ is the support chain. The candidates chains for connection with $Ch_j$, are $Ch_{k}$ and $Ch_{l}$. The angular closest chain to $Ch_j$ is the noisy $Ch_{l}$. $Ch_{k}$ is the radially closest chain to $Ch_{j}$, these means that $\|r_{j}-r_{k}\|<\|r_{j}-r_{l}\|$. Where $r_i$ is the chain's endpoint distance to the support chain. (b) Endpoint condition check. See the text for an explanation.}
   \label{fig:connectivityClosest}
\end{center}
\end{figure}


If $candidate\_chain$ satisfies the conditions, a chain in the subset $l\_no\_intersection\_j$ could be closer to $Ch_j$ in terms of the connectivity goodness conditions but at a greater angular distance. This is tested in line 9 (shown in Figure \ref{fig:connectivityClosest}.a). In angular terms, the closest chain to $Ch_j$ satisfying \Cref{equ:similiraty_criterio} is $Ch_{l}$.
However, $Ch_{k}$ exists, which is more similar but not the closest one in terms of angular distance (\Cref{equ:angular}). To fix this, we get all the chains that intersect $Ch_{l}$ and satisfy \Cref{equ:similiraty_criterio} with $Ch_j$. We sort them by radial proximity to $Ch_j$, \Cref{equ:radial}, and return the best candidate chain as the closer one regarding the radial distance. 

The \textbf{connectivity\_goodness\_condition} function is described in \Cref{algo:connectivity_goodness_condition}. From lines 1 to 4, the parameters (\Cref{tab:connectivityParameters}) are extracted from the $state$ object (an instance from \textbf{SystemStatus} object). In line 6, the chain size condition is verified and saved in $size\_condition$. In line 7, the endpoint condition is verified. Figure \ref{fig:connectivityClosest}.b shows an example of this check where $Ch_i$ is the support chain for $Ch_{i+1}$ and $Ch_{i+2}$. Endpoints $A_{i+1}$ and $B_{i+2}$ from chains $Ch_{i+1}$ and $Ch_{i+2}$ are visible. Connecting endpoints $B_{i+1}$ and $A_{i+2}$ is impossible because they do not belong to the chain support $Ch_i$ angular domain. The \Cref{equ:similiraty_criterio} condition is verified in line 8. A boolean result about the similarity condition and the absolute difference between the mean of the radial distance of the nodes associated with $Ch_j$ and $candidate\_chain$ are returned. The later is defined as $distribution\_distance = \|mean(radials_{ch_j})-mean(radials_{candidate\_chain})\|$. Finally, in line 9, all conditions are verified.
The function returns a boolean value for the conditions (the variable \textit{check}) and the value of $distribution\_distance$.

% \begin{figure*}
%    \centering
%    \includegraphics[width=0.75\linewidth]{figures/endpoint_conditions.png}
%    \caption{Endpoint condition check. See the text for an explanation.}
%    \label{fig:endpoint_condition}
% \end{figure*}


\begin{algorithm}[!htbp]
  \KwIn{$state$,\\
  $Ch_j$, // current chain\\
  $candidate\_chain$, // chain closer to $Ch_j$\\
  $Ch_i$, // support chain of $Ch_j$ and $candidate\_chain$\\
  $endpoint$, // $Ch_j$ endpoint\\
  }
\KwOut{a boolean indicating if conditions are met, $distribution\_distance$}
\SetAlgoLined
\LinesNumbered
\BlankLine 
\tcc{Parameter extraction, from \Cref{tab:connectivityParameters}}
$th\_radial\_tolerance$ $\leftarrow$ $state.th\_radial\_tolerance$ \\ 
$th\_distribution\_size$$\leftarrow$$state.th\_distribution\_size$ \\
$th\_regular\_derivative$$\leftarrow$$state.th\_regular\_derivative$ \\
$derivative\_from\_center$$\leftarrow$$state.derivative\_from\_center$ \\

\tcc{Condition checks}
$distribution\_distance$ $\leftarrow$  None\\

$size\_condition$ $\leftarrow$ $Ch_j.size$ + $candidate\_chain.size$ $\leq$ Nr\\

$endpoint\_conditions$ $\leftarrow$  check\_endpoints($Ch_i, Ch_j, candidate\_chain, endpoint$) // see  \Cref{fig:connectivityClosest}.b \\

$similarity\_condition$, $distribution\_distance$ $\leftarrow$  similarity\_conditions($state$, $th\_radial\_tolerance$,$th\_distribution\_size$, $th\_regular\_derivative$, $derivative\_from\_center$, $Ch_i$, $Ch_j$, $candidate\_chain$, $endpoint$) // \Cref{equ:similiraty_criterio}\\


$check$ $\leftarrow$ $size\_condition$ and $endpoint\_condition$ and $similarity\_condition$\\ 

\KwRet{$check$, $distribution\_distance$}
\caption{Connectivity goodness condition}
\label{algo:connectivity_goodness_condition}
\end{algorithm} 



\subsubsection{Postprocessing}

This last stage aims to complete the remaining chains, relaxing the conditions even more. At this point, many chains are closed (i.e., $size = Nr$), which we call \textit{rings}. There are some non-closed chains (noisy or part of a ring) that, for some reason, are still incomplete. We use the information on the neighborhood chains to close or discard these remaining chains. %From here on, the area between two rings is called \textit{region}. 
The ideas on connecting chains are the same as those presented in the previous section.% However, if a complete description of the algorithms is desired, it can be found in the supplementary materials section along with their code.

It can remain some chains belonging to the same ring but not forming a closed chain. Often, this is due to a minor overlapping between chains (see \Cref{fig:posprocessing_zoom}). To solve this problem, we cut the overlapping chains in such a way as to avoid intersections between them and then try to reconnect the resulting chains that respect the connectivity goodness conditions.  

Given two closed chains containing a set of chains between them, suppose the added angular length of the non-overlapping chains between the rings is greater than 180 degrees. In that case, we consider that those chains have enough information about the ring, so we complete it by interpolating between rings and using the location of the existing chains. The chains that become part of the closed chain are the ones that meet the connectivity goodness conditions using the last column of Table \ref{tab:connectivityParameters}.


 
\begin{figure*}
\begin{center}
   \includegraphics[width=0.3\linewidth]{figures/F03d_connect_selected_region}
   \includegraphics[width=0.3\linewidth]{figures/F03d_connect_zoom}
   \includegraphics[width=0.3\linewidth]{figures/F03d_posprocessing_zoom}
   \caption{a) F03d disk after the connecting stage. b) There is a ring that cannot be closed because of chain intersection issues. c) The ring is closed after the postprocessing stage.}
   \label{fig:posprocessing_zoom}
\end{center}
\end{figure*}


\subsection{Pith detection}
\label{sec:pith}
The pith position is an input for the method. Users can set it manually or using the method proposed by Decelle et al.,  \cite{ipolPith}, which is at the IPOL site.



==> CSTRD_IPOL_v1/antecedents.tex <==
\label{sec:antecedentes}

Tree ring detection is an old and essential problem in forestry with multiple uses. Due to the particularity of the species of the concerned trees, many practitioners still use a manual approach, measuring the tree rings with a ruler or other (manual) tree-ring measuring system. This is a tedious and time-consuming task.

Cerda et al. \cite{CerdaHM07} proposed a solution for detecting entire growth rings based on the Generalized Hough Transform. This work already suggests some general considerations that lead to the principal steps of our approach, as illustrated in Figure \ref{fig:algo}. The method was tested on ten images; neither the code nor the data are publicly available.

Norell \cite{Norell-2009} proposes a method to automatically compute the number of annual rings in end faces acquired in sawmill environments. The method applies the Grey Weighted Polar Distance Transform \cite{Norell2007GreyWP} to a rectangular section (core) that includes the pith and avoids knots or other disturbances.  Norell used 24 images for training and 20 for testing its method, but the images are neither publicly available nor the method's code.

Zhou et al. \cite{Zhou2012} proposed a method based on the traditionally manual approach, i.e., tracing two perpendicular lines across the slice and counting the peaks. They use a watershed-based method and show results on five discs. Neither the algorithm nor the data are available.

Henkel et al. \cite{Henke2014SemiautomaticTR} propose a semiautomatic method for detecting tree rings on full tree cross sections using an Active Contours approach. The authors report good results on several examples, but neither the data nor the algorithm is available.

Kennel et al. \cite{KennelBS15} uses the Dual-Tree Complex Wavelet Transform \cite{Kingsbury2001ComplexWF} as part of an active contour approach. This method, which works in the entire cross-section of the tree, gives very good results on seven publicly available images. We call it the Kennel dataset and try our method in this work to compare visually our results with those reported by the authors on those images. They made available their results over their dataset, but we couldn't successfully process it due errors in the files. Additionally,  code is unavailable, so it is impossible to see how it works with our data. 

Makela et al. \cite{JacobiSets} proposed an automatic method based on Jacobi Sets for the location of the pith and the ring detection on complete cross-sections of trees. Neither the code nor the data are publicly available.

\cite{DeepDendro} \cite{inbd} 

Fabijańska et al. \cite{FABIJANSKA2017279} proposed a fully automatic image-based approach for detecting tree rings over core images. The method is based on the linking of image gradient peak detected pixels and is applied over a dataset with three ring-porous wood species. The authors also proposed a deep convolutional neural network for detecting tree-rings over core images in \cite{DeepDendro}. Comparing both methods, they reported a precision of 43\% and a recall of 51\% for the classical approach, and a precision of 97\%, and a recall of 96\% for the deep learning one. Neither the code nor the data are publicly available.

Recently, Polek et al.\cite{Polek2022AutomationOT} used a machine learning-based approach for automatically detecting tree rings of coniferous species but, as most of the reviewed results, process cores instead of the whole cross-section.

This is the most common approach, and most algorithms and manual protocols use core images as input. But in some cases, as if the aim is to detect compression wood, we must mark the whole cross-section to study the asymmetries between rings.

Gillert et al, \cite{inbd} proposed a method for tree-ring detection over the whole cross-section but applied it to high-resolution images of shrub cross-sections specially conditioned for microscopy observation. They apply a deep learning approach using an Iterative Next Boundary Detection Network that, starting from the pith, infers the annual ring at each iteration step.  The method was trained and tested on images obtained under conditions that cannot be applied to cross-sections of full trees (At~\Cref{sec:inbd}, we illustrate the results of their model over our datasets). 

There exist several dendrochronology commercially available software packages. Some consist of a set of tools that help the practitioners to trace the rings manually. Others are semiautomatic, including image-processing tools to propose the ring limits. The performance generally varies significantly with particular wood anatomical features linked to wood species, climate, etc. For example, MtreeRing \cite{MtreeRing} is built using the R statistical language. It uses mathematical morphology for noise reduction and includes several methods for helping in the detection of rings (watershed-based segmentation, Canny edge detector). Like many other algorithms, it proposes an interactive tool for manual marking. To the best of our knowledge, the code is not publicly available. The CooRecorder \cite{Maxwell2021MeasuringTW}  is another software application
of this class, with several tools to help practitioners in the dendrochronological task, for example, to precisely determine the earlywood-latewood limits, using a zoom visualization and interactive tools.  Constantz et al., \cite{CONSTANTZ2021125831} develop a tool for measuring \textit{S. Paniculatum} rings. Their software measures trace by constructing transects and the rings' areas. The input for this method is a sketch image in SVG format, with some information about the center and the rings represented by polylines, produced with Adobe Illustrator.

Summing up, most of the methods or packages work on cores instead of the whole disc, or microscopic images. Moreover, the code is rarely publicly available.



==> CSTRD_IPOL_v1/antecedents_new.tex <==
\label{sec:antecedentes}

Tree ring detection is an old and essential problem in forestry, and it has multiple uses in dendroecology, dendrochronology, forest management, and other applications. Due to the species idiosyncrasies, many practitioners still use a manual approach, using a ruler or other (manual) tree-ring measuring system, which is a tedious and time-consuming task that requires an expert operator.

%Several methods exist for automatically detecting tree rings in core images \cite{Norell-2009, Norell2007GreyWP, Zhou2012, Polek2022AutomationOT}. As the core approach is more popular, most available datasets used by machine learning-based methods for training are of that type, and most deep learning-based approaches are designed for core images. 
Among the strategies proposed in recent years for the automation of tree ring delineation over wood cross-section images, we can mention the classic image-processing approaches that try to detect borders and then reconstruct the ring pattern \cite{CerdaHM07, Norell2007GreyWP, Zhou2012, Henke2014SemiautomaticTR, KennelBS15, JacobiSets} and the algorithms based on deep learning methods which try to learn the solution from the data \cite{inbd}. The core approaches are more extended, resulting in a significantly greater number of data sets. Hence, the deep learning methods are generally designed for core dendrochronology \cite{DeepDendro, Polek2022AutomationOT}. 

%Among the methods based on ring pattern reconstruction
%Among the ring delineation methods on cross-section images based on pattern recognition, 
Cerda et al. \cite{CerdaHM07} proposed a classic image processing approach for detecting entire growth rings based on the Generalized Hough Transform. This work already suggests using the general geometrical structure of the tree rings, which we use in our approach, as illustrated in Figure \ref{fig:algo}. Norell et al. use the Grey Weighted Polar Distance Transform \cite{Norell2007GreyWP} to process end faces acquired in sawmill environments. Still, the method implies using rectangular sections, including the pith, and avoiding knots or other disturbances, diminishing the generality of the approach. Zhou proposes a much simpler method \cite{Zhou2012}, which resembles the traditional manual procedure in which two perpendicular lines across the slice are traced. The watershed method is applied to the profiles to obtain the peaks corresponding to each ring. Henkel et al. use an active contours approach \cite{Henke2014SemiautomaticTR} alone or coupled with a Dual-Tree Complex Wavelet Transform \cite{KennelBS15} based on the evolution of a partial differential equation that includes terms related to the image content and to the curve itself. Many PDE-based algorithms are time-consuming, making them difficult to use in real-time applications. Makela et al. proposed a method based on Jacobi Sets to detect the ring pattern and pith location \cite{JacobiSets}. All these methods rely on detecting the edges corresponding to the tree rings and different strategies to reconstruct the pattern. In all cases, the pith is the center of a general structure. Most of these works were tested against a few images (ranging from 7 to 20). Unfortunately, the code and used images are unavailable in these cases for testing and comparing the results with other methodologies.

Deep learning approaches have become more popular in recent years and have naturally been applied to this problem. Still, the scarcity of labeled data for a given species is a significant problem in the area, as the methods must be tailored to the particularities of each species. Gillert et al., \cite{inbd} proposed a method for cross-section tree-ring detection named Iterative Next Boundary Detection Network (INBD) but applied it to high-resolution images of shrub cross-sections specially conditioned for microscopy observation. In this case, the images are not only of a particular species, but also the microscopic resolution introduces specific characteristics. Starting from the pith, the method infers the annual ring at each iteration step, detecting ring by ring from the medulla to the tree's bark. A problem can arise if an intermediate ring is badly processed. In those cases, the error propagates and affects all the rings outward. The method was trained and tested on images obtained under the specific conditions of microscopic images of shrub species. This is the unique method for which we have access to the code, allowing us to compare it with our approach. In \Cref{sec:inbd}, we illustrate the results of applying their model to our datasets, training their method for our particular images. 

Besides the INBD method, most deep-learning-based approaches are applied to core images. For example, recently, Polek et al.\cite{Polek2022AutomationOT} applied a deep learning approach to process cores of coniferous species. Fabijańska et al. proposed both a classic image-processing approach \cite{FABIJANSKA2017279} (based on the linking of image gradient peak detected pixels) and a convolutional neural network one \cite{DeepDendro} for detecting tree rings over core images. Comparing both methods, they reported a precision of 43\% and a recall of 51\% for the classical approach, a precision of 97\%, and a recall of 96\% for the deep learning one. Without the code or the data, it is impossible to verify these claims with other species or datasets (their experiments concern three ring-porous wood species).

In short, deep learning-based methods are almost all for cores, and the absence of labeled databases makes it difficult to use them on complete slices. Classical methods are generally based on edge detection and build rings out of them. Most reported methods lack the code or the data to verify their claims. Still, their analysis leads to the assumption that the presence of perturbations such as fungus, cracks, and knots strongly affects the performance because the construction of each ring depends on the previous ones. Therefore, an error in the pith or rings close to the center propagates to the rest of the structure.


 

==> CSTRD_IPOL_v1/conclusions.tex <==
\label{sec:conclusions}

We presented an automatic method for Tree Ring Detection of cross-section wood images. It achieves an F-Score of 97\% in the Kennel dataset and 89\% in the more complex UruDendro dataset. The CS-TRD method outperforms deep learning state-of-the-art methods such as the INBD \cite{inbd} in the Pinus taeda species. It performs well even in the presence of fungus, cracks, and knots and in two different species (Abies alba and Pinus taeda).

The method runs at an average execution time of 17 seconds in the UruDendro dataset and 11 seconds in the Kennel dataset on an Intel Core i5 10300H workstation with 16 GB of RAM (without GPU). Compared with the time each annotator needs to manually delineate every disk, 3 hours on average, is a vast improvement. CS-TRD can be fully implemented in C++ to accelerate the execution time compared to the Python implementation\footnote{https://medium.com/agents-and-robots/the-bitter-truth-python-3-11-vs-cython-vs-c-performance-for-simulations-babc85cdfef5}. This will allow using the method in real-time applications.

In the future, we plan to include the  automatic pith detection, % \cite{marichal2024automaticPithDetector}
 extend the method to other tree species, and explore machine-learning techniques to improve the results.

%We presented an automatic method (besides the pith detection, for which an automatic algorithm exists \cite{ipolPith} Y EL NUESTRO?) for Tree Ring Detection of cross-section wood images, which achieves an F-Score of 97\% in the Kennel dataset and an F-Score of 89\% in the (more complex) UruDendro dataset. CS-TRD method outperforms state-of-the-art methods such as the INBD (\cite{inbd}) in the Pinus taeda species. CS-TRD has good performance even in the presence of fungus, cracks, and knots, as well as in two species (Abies alba and Pinus taeda).

%The method runs at an average execution time of 17 seconds in the UruDendro dataset and 11 seconds in the Kennel dataset on an Intel Core i5 10300H workstation with 16 GB of RAM (without GPU). Compared with the time each annotator needs to delineate every disk, 3 hours on average manually is a vast improvement. The CS-TRD method can be fully implemented in C++ to accelerate the execution time compared to the Python implementation\footnote{https://medium.com/agents-and-robots/the-bitter-truth-python-3-11-vs-cython-vs-c-performance-for-simulations-babc85cdfef5}. This will allow using the method in real-time applications.

%As far as we know, it is the first automatic method for detecting tree rings on whole cross sections with available code.

%In the future, we will include the automatic detection of the pith \cite{nuestropaperpth}, extend the method to other tree species, and explore machine-learning techniques to learn the pattern in the data. ESTA ULTIMA FRASE NO SE SI TIENE SENTIDO, ...

==> CSTRD_IPOL_v1/dataset.tex <==
\section{Datasets}
\label{sec:database}

To test the proposed method, we use two datasets:
\begin{enumerate}
    \item The \textbf{Kennel} dataset. Kennel et al. \cite{KennelBS15} made available a public dataset of 7 images of Abies alba and presented a method for detecting tree rings. We were unable to process the annotations given by the authors. The characteristics of this dataset are described in \Cref{tab:KennelDataset}. We label the dataset with the same procedure as the UruDendro dataset to evaluate the results.
    \item  The \textbf{UruDendro} dataset. An online database \cite{UruDendro} with images of cross-sections of commercially grown \textit{Pinus taeda} trees from northern Uruguay, ranging from 13 to 24 years old, composed of fourteen individual trees collected in February 2020 in Uruguay.  Seven trees correspond to a lumber company (denoted by the letter F), and the other seven correspond to a plywood company (denoted by the letter L).  Each company applied different silviculture practices. 
    The individuals were identified by the letter of the company, a two-digit number, and a lowercase letter corresponding to the height where each cross-section was obtained. Heights were coded as follows: a = 10 cm above the ground, b = 165 cm, c = 200 cm, d = 400 cm, and e = 435 cm.
    The cross-sections were about 5 to 20 cm thick and were dried at room temperature without further preparation.  As a consequence of the drying process, radial cracks and blue fungus stains were developed in the cross-sections. Surfaces were smoothed with a handheld planer and a rotary sander. Photographs were taken under different lighting conditions; cross-sections a, b, and e were photographed indoors and moistened to maximize contrast between early- and late-wood.  Pictures of dry cross-sections c and d were taken outdoors.  
    The dataset has 64 images of different resolutions, described in \Cref{tab:uruguayDataset}. The collection contains several challenging features for automatic ring detection, including illumination and surface preparation variation, fungal infection (blue stains), knot formation, missing bark and interruptions in outer rings, and radial cracking.  The proposed CS-TRD tree-ring detection method was checked against manual delineation of all rings by users of varying expertise using the Labelme tool \cite{wada}. At least two experts annotate all images. 
    Figure \ref{fig:ddbb} shows some images in this UruDendro dataset. 
\end{enumerate}

\begin{table}[htbp]
\centering
\caption{The Kennel dataset, with the name and dimensions of each image, the number of expert marks, and the number of rings in each one.}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Image} & \textbf{Marks} & \textbf{Rings} & \textbf{Height  (pixels)} & \textbf{Width  (pixels)} \\ \hline
\textbf{AbiesAlba1} & 4 & 52 & 1280 & 1280 \\ \hline
\textbf{AbiesAlba2} & 2 & 22 & 1280 & 1280 \\ \hline
\textbf{AbiesAlba3} & 3 & 27 & 1280 & 1280 \\ \hline
\textbf{AbiesAlba4} & 1 & 12 & 1024 & 1024 \\ \hline
\textbf{AbiesAlba5} & 3 & 30 & 1280 & 1280 \\ \hline
\textbf{AbiesAlba6} & 2 & 21 & 1280 & 1280 \\ \hline
\textbf{AbiesAlba7} & 1 & 48 & 1280 & 1280 \\ \hline
\end{tabular}
\label{tab:KennelDataset}
\end{table}

\begin{table}[htbp]
\centering
\scriptsize
\caption{The UruDendro dataset, with the name and dimensions of each image, the number of expert marks, and the number of rings in each one.}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Image} & \textbf{Marks} & \textbf{Rings} & \textbf{Height (pixels)} & \textbf{Width (pixels)} \\ \hline
\textbf{F02a} & 2 & 23 & 2364 & 2364 \\ \hline
\textbf{F02b} & 2 & 22 & 1644 & 1644 \\ \hline
\textbf{F02c} & 4 & 22 & 2424 & 2408 \\ \hline
\textbf{F02d} & 2 & 20 & 2288 & 2216 \\ \hline
\textbf{F02e} & 2 & 20 & 2082 & 2082 \\ \hline
\textbf{F03a} & 2 & 24 & 2514 & 2514 \\ \hline
\textbf{F03b} & 2 & 23 & 1794 & 1794 \\ \hline
\textbf{F03c} & 1 & 24 & 2528 & 2596 \\ \hline
\textbf{F03d} & 1 & 21 & 2476 & 2504 \\ \hline
\textbf{F03e} & 3 & 21 & 1961 & 1961 \\ \hline
\textbf{F04a} & 2 & 24 & 2478 & 2478 \\ \hline
\textbf{F04b} & 1 & 23 & 1760 & 1762 \\ \hline
\textbf{F04c} & 3 & 21 & 913 & 900 \\ \hline
\textbf{F04d} & 2 & 21 & 921 & 899 \\ \hline
\textbf{F04e} & 1 & 21 & 2070 & 2072 \\ \hline
\textbf{F07a} & 1 & 24 & 2400 & 2400 \\ \hline
\textbf{F07b} & 3 & 23 & 1740 & 1740 \\ \hline
\textbf{F07c} & 1 & 23 & 978 & 900 \\ \hline
\textbf{F07d} & 1 & 22 & 997 & 900 \\ \hline
\textbf{F07e} & 1 & 22 & 2034 & 2034 \\ \hline
\textbf{F08a} & 3 & 24 & 2383 & 2383 \\ \hline
\textbf{F08b} & 2 & 23 & 1776 & 1776 \\ \hline
\textbf{F08c} & 2 & 23 & 2624 & 2736 \\ \hline
\textbf{F08d} & 2 & 22 & 2388 & 2400 \\ \hline
\textbf{F08e} & 2 & 22 & 1902 & 1902 \\ \hline
\textbf{F09a} & 1 & 24 & 2106 & 2106 \\ \hline
\textbf{F09b} & 4 & 23 & 1858 & 1858 \\ \hline
\textbf{F09c} & 1 & 24 & 2370 & 2343 \\ \hline
\textbf{F09d} & 1 & 23 & 2256 & 2288 \\ \hline
\textbf{F09e} & 1 & 22 & 1610 & 1609 \\ \hline
\textbf{F10a} & 2 & 22 & 2136 & 2136 \\ \hline
\textbf{F10b} & 2 & 22 & 1677 & 1677 \\ \hline
\textbf{F10e} & 1 & 20 & 1800 & 1800 \\ \hline
\textbf{L02a} & 1 & 16 & 2088 & 2088 \\ \hline
\textbf{L02b} & 3 & 15 & 1842 & 1842 \\ \hline
\textbf{L02c} & 1 & 13 & 1016 & 900 \\ \hline
\textbf{L02d} & 2 & 14 & 921 & 900 \\ \hline
\textbf{L02e} & 2 & 14 & 1914 & 1914 \\ \hline
\textbf{L03a} & 2 & 17 & 2296 & 2296 \\ \hline
\textbf{L03b} & 2 & 16 & 2088 & 2088 \\ \hline
\textbf{L03c} & 2 & 16 & 2400 & 2416 \\ \hline
\textbf{L03d} & 2 & 16 & 2503 & 2436 \\ \hline
\textbf{L03e} & 2 & 14 & 1944 & 1944 \\ \hline
\textbf{L04a} & 4 & 17 & 2418 & 2418 \\ \hline
\textbf{L04b} & 2 & 16 & 1986 & 1986 \\ \hline
\textbf{L04c} & 2 & 16 & 2728 & 2704 \\ \hline
\textbf{L04d} & 2 & 16 & 2544 & 2512 \\ \hline
\textbf{L04e} & 1 & 15 & 1992 & 1992 \\ \hline
\textbf{L07a} & 2 & 17 & 2328 & 2328 \\ \hline
\textbf{L07b} & 2 & 16 & 2118 & 2118 \\ \hline
\textbf{L07c} & 3 & 17 & 2492 & 2481 \\ \hline
\textbf{L07d} & 1 & 16 & 2480 & 2456 \\ \hline
\textbf{L07e} & 2 & 15 & 1980 & 1980 \\ \hline
\textbf{L08a} & 2 & 17 & 2268 & 2268 \\ \hline
\textbf{L08b} & 2 & 16 & 1836 & 1836 \\ \hline
\textbf{L08c} & 1 & 16 & 2877 & 2736 \\ \hline
\textbf{L08d} & 2 & 14 & 2707 & 2736 \\ \hline
\textbf{L08e} & 1 & 15 & 1666 & 1666 \\ \hline
\textbf{L09a} & 1 & 17 & 1963 & 1964 \\ \hline
\textbf{L09b} & 3 & 16 & 1802 & 1802 \\ \hline
\textbf{L09c} & 1 & 16 & 943 & 897 \\ \hline
\textbf{L09d} & 2 & 15 & 1006 & 900 \\ \hline
\textbf{L09e} & 1 & 15 & 1662 & 1662 \\ \hline
\textbf{L11b} & 4 & 16 & 1800 & 1800 \\ \hline
\end{tabular}
\label{tab:uruguayDataset}
\end{table}





==> CSTRD_IPOL_v1/experiments.tex <==
\label{sec:ExperimentsAndResults}

\subsection{Datasets}
\label{sec:database}

We use two datasets to evaluate the CS-TRD method. 

The first one (\textbf{UruDendro}) is an online database \cite{UruDendro} with images of cross-sections of fourteen commercially grown \textit{Pinus taeda} trees from northern Uruguay. These trees are 13 to 24 years old and were collected in February 2020. The cross-sections are between 5 and 20 cm thick and were dried at room temperature without further preparation, which resulted in the development of radial cracks and blue fungus stains. Surfaces were smoothed with a handheld planer and a rotary sander. The dataset consists of 64 images of different resolutions, ranging between 1000 and 3000 pixels in width. It contains challenging features for automatic ring detection, including varying illumination and surface preparation, fungal infection (blue stains), knots, missing bark and interruptions in outer rings, and radial cracking. At least two experts annotate the images using the Labelme tool \cite{wada}. Figure \ref{fig:ddbb} shows some images from the dataset. 

The second dataset (\textbf{Kennel}) is proposed in \cite{KennelBS15}, which made available a public set of 7 (1280x1280 pixels) images of Abies alba along with a method for detecting tree rings (the code is not available). We labeled the dataset with the same procedure as the \textbf{UruDendro} dataset as we could not process the annotations given by the authors.


\subsection{Metrics}
\label{sec:metric}
To assess the method, we developed a metric based on the one proposed by Kennel et al. \cite{KennelBS15}. To determine if a ring is detected, we define a ring influence area as the set of pixels closer to that ring. For each ray, the frontier is the midpoint between the nodes of consecutive ground truth (GT) rings. \Cref{fig:influece_area}.b show the influence area for rings in disk F03d. %Each GT ring is depicted in black and is the center of its influence area. 
\Cref{fig:influece_area}.a shows the detections (in red) and GT marks (in green) for the same image.

\begin{figure*}
\begin{centering}
    \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=\textwidth]{figures/f03d_dt_and_gt.png}
%    \label{fig:dtvsgt}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=\textwidth]{figures/f03d_areas_influencia.png}
%    \label{fig:influence}
    \caption{}
    \end{subfigure}
       \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=\textwidth]{figures/f03d_polar_heat_map.png}
%    \label{fig:error}
    \caption{}
    \end{subfigure}
   \caption{Measuring the error of automatic detections for image F03d: (a) In green, the GT; in red, the detections produced by the method. (b) Areas of influence of the GT rings. (c) Absolute error, in pixels, between the detections and the GT.}
   \label{fig:influece_area}
\end{centering}
\end{figure*}

The influence region associates a detected curve with a GT ring. In both cases, nodes are associated with the $N_r$ rays. Given a GT ring, we assign it to the nearest detection using:

\begin{equation}
    Dist = \sqrt{\frac{1}{N_r}\sum_{i=0}^{N_r-1}\left(dt_i-gt_i\right)^2}\hspace{0.5cm} 
    \label{equ:rmse}
\end{equation}

Where $i$ represents the ray direction, $dt_i$ is the radial distance (\Cref{equ:radial}) of detected node $i$, and $gt_i$ is the radial distance (\Cref{equ:radial}) of the corresponding GT node $i$. 

The closest detection may be far from the corresponding GT ring. To match a detected curve with a GT ring, it is essential to ensure that the identified chain is the closest one to the ring and that it is sufficiently close. We utilize the influence area of each GT ring (\Cref{fig:influece_area}.b). Upon detecting a curve, if the proportion of nodes within that chain that falls within the influence area of the nearest ring exceeds a specified threshold parameter ($th\_pre=60\%$, see \Cref{sec:precisionTrheshold}), we assign the detected curve to the corresponding GT ring. If it falls below the threshold, the detection is not associated with any GT ring. In other words, for a detected curve to be assigned to a GT ring and considered a true positive, at least 60\% of its nodes must be within the influence area of that GT ring.

We define the absolute error $A\epsilon_i$ (in pixels) for the \textit{node} $i$ as the absolute difference in pixels between the GT ring and the detected ring associated with it:

$$
A\epsilon_i = |r^d_i - r^{GT}_i|
$$

Where $r^d_i$ is the radial distance from the center to node $i$ of the detected ring, and $r^{GT}_i$ is the same for the GT ring. Figure \ref{fig:influece_area}.c shows the absolute error between the GT and the detected rings assigned to them. Red represents a low error, while yellow, green, and blue represent a higher error. As can be seen, the error is concentrated around the knot, affecting the precise detection of some rings.

Once all the detected chains are matched with the GT rings, we calculate the following values:
\begin{enumerate}
    \item True Positive (TP): when the identified closed chain and the GT ring match.
    \item False Positive (FP): when the identified closed chain doesn't match any GT ring.
    \item False Negative (FN): when a GT ring doesn't match any detected closed chain.
\end{enumerate}

Precision is given by $P=\frac{TP}{TP+FP}$, Recall by
$R=\frac{TP}{TP+FN}$ and the F-Score by $F=\frac{2PR}{P+R}$. 


\subsection{Experiments}
\label{sec:experiments}

This section presents some experiments to help us better understand the method and its limitations. % the end of the section, an experiment shows how the results depend on the metric threshold $ th_{pre}$. 

\Cref{tab:best_res} presents the metric results for the optimal values of $\sigma$ and image resolution on both datasets. For example, CS-TRD fails to detect one ring in the image \textit{F03d} ($FN=1$), and the other rings are correctly detected, leading to the displayed values of $P$, $R$, and $F$. The table also compares the mean execution time by image and the RMSE error in pixels (\Cref{equ:rmse}) between the detected and GT rings. All experiments used an Intel Core i5 10300H workstation with 16GB of RAM. These are very good results, considering the data diversity and the presence of perturbations.


\begin{table}[!ht]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
Dataset                                          & \multicolumn{1}{l|}{Image Size (pixels)} & \multicolumn{1}{l|}{$\sigma$} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{F} & \multicolumn{1}{l|}{RMSE} & \multicolumn{1}{l|}{Execution Time (sec.)} \\ \hline
UruDendro & 1500x1500 & 3.0 & 0,95 & 0,86 & 0,89 & 5.27 & 17.3 \\ \hline
Kennel & 1500x1500  & 2.5 & 0,97 & 0,97 & 0,97 & 2.4  & 11.1   \\ \hline
\end{tabular}
\caption{Mean performance and execution time for both datasets' at the optimal $\sigma$ and image resolution.}
\label{tab:best_res}
\end{table}


\subsubsection{Edge detector optimization stage}
\label{exp:size}
The algorithm heavily relies on the edge detector stage. In the first experiment, we test different $\sigma$ values for the Canny Devernay edge detector to get the one that maximizes the F-Score for the UruDendro dataset. This dataset shows significant variations in image resolution, allowing us to study the overall performance with different input image dimensions. The results are presented in Figures \ref{fig:sigma-results_ac}.a and \ref{fig:sigma-results_ac}.b. We compute the average F-Score for the original image sizes and then scale all images in the dataset to $640\times640$, $1000\times1000$, and $1500\times1500$ pixels. The best result was achieved for the size $1500\times1500$ with $\sigma=3.0$. The execution time varies with the image size. The average execution time for the $1500\times1500$ size is 17 seconds. The execution time decreased as $\sigma$ increased because fewer edge chains were detected. Results for the same experiment on the Kennel dataset are shown in Figures \ref{fig:sigma-results_ac}.c and \ref{fig:sigma-results_ac}.d. The best F-Score is achieved for the $1500\times1500$ resolution with $\sigma=2.5$. The lower optimal $\sigma$ value can be attributed to the Kennel dataset having images with more rings on the disk, averaging 30 rings. In comparison, the UruDendro one has 19 rings per disk on average. Table \ref{tab:best_res} summarizes the results of this experiment.

\begin{figure*}[ht]
\begin{centering}
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/fscore-sigma.png}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/exec_time.png}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/fscore-sigma_ac.png}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/exec_time_ac.png}
    \caption{}
    \end{subfigure}
   \caption{ Influence of the image size and edge detector $\sigma$ parameter experiment. Each curve represents a different image resolution: $640\times640$, $1000\times1000$, $1500\times1500$, and the original resolution (in blue). (a) Average F1 vs. $\sigma$ for different image sizes over the UruDendro dataset. (b) Average execution time (in seconds) vs $\sigma$ for different image sizes over the UruDendro dataset. (c) Average F1 vs. $\sigma$ for different image sizes over the Kennel dataset. (d) Average execution time (in seconds) vs $\sigma$ for different image sizes over the Kennel dataset.
   }
   \label{fig:sigma-results_ac}
\end{centering}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%% table with results
\subsubsection{Pith position sensibility}
The next experiment assesses the method's sensitivity to errors in the pith estimation. \Cref{fig:average_pith_position_exp}.a shows 48 different pith positions used in this experiment (eight different pith positions across six rays). These radially displaced pith positions are selected as follows:
\begin{itemize}
    \item We define an error step along a ray as 25\% of the first ring equivalent diameter.
    \item Three positions are marked inside ring 1, with errors  25\%, 50\%, and 75\% off the GT center in the ray direction.
    \item One position is marked on ring 1.
    \item Three positions are marked between the first and second rings, with the same increasing errors in the ray direction.
    \item Finally, another position is marked on ring 2.
\end{itemize}

We executed the algorithm for each disk and pith position of the UruDendro dataset (size of $1500\times1500$ and $\sigma=3.0$), resulting in 48 outcomes. We calculated the average RMSE and F-Score measurements for the six-ray directions for each radially displaced pith position. This produced two eight-coordinate vectors, one for RMSE and one for the F-Score. Figures \ref{fig:average_pith_position_exp}.b and \ref{fig:average_pith_position_exp}.c illustrates the average F-Score and RMSE for each error position across the dataset, respectively. The F-Score decreases as the error in the pith estimation increases, while the RMSE is less sensitive to pith errors.
 
%\begin{figure*}
%\begin{centering}
%\includegraphics[width=0.3\textwidth]{figures/zoom_pith_experiment.png}
%\caption{Pith position experiment. Given six ray directions, eight different pith positions are marked. The method is executed for each marked pith position. GT rings are marked in green}
%\label{fig:pith_sensitivity}
%\end{centering}
%\end{figure*}


\subsubsection{Metric precision threshold}
\label{sec:precisionTrheshold}
In this experiment, we examine how performance changes with different values of the $th\_pre$ parameter, which determines the number of ring nodes within the influence area to be considered in the detection-to-ground-truth assignation step. Figure \ref{fig:metric_our_database_ac} displays the results for the UruDendro and Kennel datasets. As anticipated, higher precision leads to lower RMSE but lower F-Score. Based on these findings, we fixed $th\_pre = 60\%$ as the default value, which appears to be a good compromise.

\begin{figure*}
\begin{centering}
   \begin{subfigure}{0.28\textwidth}
   \includegraphics[width=\textwidth]{figures/zoom_pith_experiment.png}
    \caption{Pith position grid}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/pith_position_experiment_f1.png}
    \caption{Average F-Score over the UruDendro dataset.}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/pith_position_experiment_rmse.png}
    \caption{Average RMSE over the  UruDendro dataset.}
    \end{subfigure}
   \caption{Pith position experiment. (a) Eight different pith positions are marked given six ray directions. We executed the method for each marked pith position. GT rings are in green. (b and c) For each disk of the UruDendro dataset, we run the method using the 48 different pith positions. Results are averaged over the six rays' directions per error position. The X-axis values correspond to increments of 25 \% in error, i.e., the value 2 implies an error of 50 \% of the first ring equivalent diameter in the pith position concerning the GT.}
   \label{fig:average_pith_position_exp}
\end{centering}
\end{figure*}


%In this experiment, we see how the performance varies with different values of $th\_pre$. This parameter controls the number of nodes of the ring that lie within the Influence Area to be considered in the detection-to-ground-truth assignation step. Figure \ref{fig:metric_our_database} and Figure \ref{fig:metric_our_database_ac} show results for UruDendro and Kennel datasets, respectively. As expected, higher precision implies lower (better) RMSE but lower F-Score. Given these results, we fix $th\_pre=60\%$ as a default value, which seems a good compromise.

\begin{figure*}[ht]
\begin{centering}
    \begin{subfigure}{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/metric_fscore.png}
 %   \caption{}
%    \label{fig:metric_our_database_F-Score}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/metric_rmse.png}
  %  \caption{}
 %   \label{fig:metric_our_database_rmse}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/metric_fscore_ac.png}
   % \caption{}
 %   \label{fig:metric_our_database_F-Score_ac}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
    \includegraphics[width=\textwidth]{figures/metric_rmse_ca.png}
   % \caption{}
 %   \label{fig:metric_our_database_rmse_ac}
    \end{subfigure}
   \caption{Performance metrics were computed for different values of the $th\_pre$ parameter. The first row shows the results for the Urudendro dataset, and the second row for the Kennel dataset. The left column shows the average F-Score, and the right column shows the average RMSE.}
   \label{fig:metric_our_database_ac}
\end{centering}
\end{figure*}






\subsection{Results}
\label{sec:results}
This section provides a quantitative analysis of the CS-TRD method performance on challenging images in the datasets. \Cref{fig:ddbb_output} illustrates some results of the CS-TRD over the UruDendro dataset. Note the successful performance of CS-TRD on disks with cracks (F02b), knots (L03c), and fungus (L02b). The mean F-Score for the whole dataset is 0.89 (\Cref{tab:best_res}), indicating the successful detection of rings in complex images containing knots, fungus, and cracks.  Results of the CS-TRD algorithm on other samples of the Urudendro dataset are in the supplemental material. %The algorithm demonstrates a high ring detection rate for disks F02a, F02b, F02c, F02d, F02e, F03c, and L03c. Additionally, it successfully detects rings over cracks (disks F02a, F02b, and F02e) and knots (disk L03c).
% Arrancar describiendo cualitativamente los resultados sobre UruDendro. Numericamente y los casos bordes dificiles
% Seguir por la base de Kennel

\begin{figure*}[h!]
\begin{centering}
%    \begin{subfigure}{0.3\textwidth}
%    \includegraphics[width=\textwidth]{figures/F02a_output}
%    \caption{F02a}
%    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/F02b_output}
    \caption{F02b}
    \end{subfigure}
%    \begin{subfigure}{0.3\textwidth}
%    \includegraphics[width=\textwidth]{figures/F02c_output}
%    \caption{F02c}
%    \end{subfigure}
%    \begin{subfigure}{0.3\textwidth}
%   \includegraphics[width=\textwidth]{figures/F02d_output}
%    \caption{F02d}
%    \end{subfigure}
%    \begin{subfigure}{0.3\textwidth}
%   \includegraphics[width=\textwidth]{figures/F02e_output}
%    \caption{F02e}
%    \end{subfigure}
%    \begin{subfigure}{0.3\textwidth}
%   \includegraphics[width=\textwidth]{figures/F03c_output}
%    \caption{F03c}
%    \end{subfigure}
%    \begin{subfigure}{0.3\textwidth}
%    \includegraphics[width=\textwidth]{figures/L03c_output}
%    \caption{L03c}
%    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/F07b_output}
    \caption{F07b}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{L02b_output}
    \caption{L02b}
    \end{subfigure}
   \caption{The CS-TRD method predicted detections (shown as blue curves) in some images of the UruDendro dataset.}
   \label{fig:ddbb_output}
\end{centering}
\end{figure*}




 %The results for the UruDendro dataset are shown in \Cref{Tab:results_nuestra-60}. The mean F-Score is lower, 0.89, but the images in this dataset are much more complex and include knots, fungus, and cracks. 

% \begin{table}[htbp]
% \scriptsize
% \centering
% \caption{Results on the Kennel dataset with  $th\_pre=60$. Images resized to 1500x1500 and edge detector parameter $\sigma=2.5$}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Name} & \textbf{TP} & \textbf{FP} & \textbf{TN} & \textbf{FN} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{RMSE} & \textbf{Time (sec.)} \\ \hline
% AbiesAlba1 & 49 & 1  & 0  & 3  & 0.98 & 0.94 & 0.96 & 3.66 & 18.01      \\ \hline
% AbiesAlba2 & 20 & 0  & 0  & 2  & 1.00 & 0.91 & 0.95 & 0.95 & 9.21       \\\hline
% AbiesAlba3 & 26 & 1  & 0  & 1  & 0.96 & 0.96 & 0.96 & 1.30 & 8.93       \\\hline
% AbiesAlba4 & 11 & 0  & 0  & 1  & 1.00 & 0.92 & 0.96 & 5.88 & 8.96       \\\hline
% AbiesAlba5 & 30 & 1  & 0  & 0  & 0.97 & 1.00 & 0.98 & 1.29 & 9.06       \\\hline
% AbiesAlba6 & 20 & 0  & 0  & 1  & 1.00 & 0.95 & 0.98 & 1.26 & 7.63       \\\hline
% AbiesAlba7 & 45 & 0  & 0  & 3  & 1.00 & 0.94 & 0.97 & 3.58 & 13.78 \\\hline
% Average & & & &  &0.99& 0.95& 0.97& 2.56 & 10.80 \\\hline
% \end{tabular}
% \label{tab:resultsKennel}
% \end{table}


% \begin{table}[htbp]
% %\resizebox{0.9\linewidth}{!}{
% \scriptsize
% \centering
% \caption{Results over our dataset with  $th\_pre=60\%$. Images resized to 1500x1500 and edge detector parameter  $\sigma =3$. }
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|} 
% \hline
% \textbf{Name} & \textbf{TP} & \textbf{FP} & \textbf{TN} & \textbf{FN} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{RMSE} & \textbf{Time (sec.)} \\ 
% \hline
% F10b    & 19 & 2  & 0  & 3  & 0.91 & 0.86 & 0.88 & 4.75          & 20.39       \\ 
% \hline
% F10a    & 17 & 1  & 0  & 5  & 0.94 & 0.77 & 0.85 & 4.24          & 15.23       \\ 
% \hline
% F10e    & 18 & 0  & 0  & 2  & 1.00 & 0.90 & 0.95 & 2.13          & 12.57       \\ 
% \hline
% F02c    & 21 & 0  & 0  & 1  & 1.00 & 0.96 & 0.98 & 3.76          & 12.26       \\ 
% \hline
% F02b    & 21 & 1  & 0  & 1  & 0.96 & 0.96 & 0.96 & 4.02          & 13.26       \\ 
% \hline
% F02a    & 20 & 0  & 0  & 3  & 1.00 & 0.87 & 0.93 & 1.50          & 15.29       \\ 
% \hline
% F02d    & 20 & 1  & 0  & 0  & 0.95 & 1.00 & 0.98 & 2.11          & 8.34        \\ 
% \hline
% F02e    & 20 & 1  & 0  & 0  & 0.95 & 1.00 & 0.98 & 7.62          & 23.31       \\ 
% \hline
% F03c    & 23 & 0  & 0  & 1  & 1.00 & 0.96 & 0.98 & 10.69         & 7.34        \\ 
% \hline
% F03b    & 20 & 0  & 0  & 3  & 1.00 & 0.87 & 0.93 & 2.15          & 13.95       \\ 
% \hline
% F03a    & 22 & 2  & 0  & 2  & 0.92 & 0.92 & 0.92 & 8.11          & 19.37       \\ 
% \hline
% F03d    & 19 & 1  & 0  & 2  & 0.95 & 0.91 & 0.93 & 7.81          & 11.26       \\ 
% \hline
% F03e    & 20 & 2  & 0  & 1  & 0.91 & 0.95 & 0.93 & 1.66          & 15.70       \\ 
% \hline
% F04c    & 18 & 1  & 0  & 3  & 0.95 & 0.86 & 0.90 & 5.60          & 26.88       \\ 
% \hline
% F04b    & 19 & 0  & 0  & 4  & 1.00 & 0.83 & 0.91 & 4.60          & 40.24       \\ 
% \hline
% F04a    & 21 & 1  & 0  & 3  & 0.96 & 0.88 & 0.91 & 7.71          & 28.90       \\ 
% \hline
% F04d    & 17 & 3  & 0  & 4  & 0.85 & 0.81 & 0.83 & 2.90          & 55.38       \\ 
% \hline
% F04e    & 19 & 2  & 0  & 2  & 0.91 & 0.91 & 0.91 & 9.94          & 24.33       \\ 
% \hline
% F07c    & 20 & 2  & 0  & 3  & 0.91 & 0.87 & 0.89 & 4.85          & 35.81       \\ 
% \hline
% F07b    & 17 & 3  & 0  & 6  & 0.85 & 0.74 & 0.79 & 7.99          & 45.74       \\ 
% \hline
% F07a    & 18 & 1  & 0  & 6  & 0.95 & 0.75 & 0.84 & 11.68         & 18.27       \\ 
% \hline
% F07d    & 20 & 0  & 0  & 2  & 1.00 & 0.91 & 0.95 & 1.04          & 19.95       \\ 
% \hline
% F07e    & 8  & 4  & 0  & 14 & 0.67 & 0.36 & 0.47 & 8.17          & 40.29       \\ 
% \hline
% F08c    & 21 & 1  & 0  & 2  & 0.96 & 0.91 & 0.93 & 2.05          & 13.25       \\ 
% \hline
% F08b    & 21 & 1  & 0  & 2  & 0.96 & 0.91 & 0.93 & 1.72          & 23.57       \\ 
% \hline
% F08a    & 21 & 1  & 0  & 3  & 0.96 & 0.88 & 0.91 & 5.28          & 17.13       \\ 
% \hline
% F08d    & 20 & 0  & 0  & 2  & 1.00 & 0.91 & 0.95 & 2.10          & 9.54        \\ 
% \hline
% F08e    & 22 & 0  & 0  & 0  & 1.00 & 1.00 & 1.00 & 6.70          & 17.65       \\ 
% \hline
% F09c    & 21 & 0  & 0  & 3  & 1.00 & 0.88 & 0.93 & 2.83          & 9.11        \\ 
% \hline
% F09b    & 22 & 1  & 0  & 1  & 0.96 & 0.96 & 0.96 & 2.91          & 11.98       \\ 
% \hline
% F09a    & 21 & 0  & 0  & 3  & 1.00 & 0.88 & 0.93 & 2.20          & 16.13       \\ 
% \hline
% F09e    & 14 & 5  & 0  & 8  & 0.74 & 0.64 & 0.68 & 7.08          & 38.73       \\ 
% \hline
% L11b    & 15 & 1  & 0  & 1  & 0.94 & 0.94 & 0.94 & 1.54          & 10.96       \\ 
% \hline
% L02c    & 11 & 0  & 0  & 2  & 1.00 & 0.85 & 0.92 & 5.33          & 21.33       \\ 
% \hline
% L02b    & 4  & 2  & 0  & 11 & 0.67 & 0.27 & 0.38 & 9.41          & 21.90       \\ 
% \hline
% L02a    & 14 & 1  & 0  & 2  & 0.93 & 0.88 & 0.90 & 16.95         & 26.21       \\ 
% \hline
% L02d    & 7  & 3  & 0  & 7  & 0.70 & 0.50 & 0.58 & 5.66          & 28.80       \\ 
% \hline
% L02e    & 11 & 0  & 0  & 3  & 1.00 & 0.79 & 0.88 & 4.92          & 18.66       \\ 
% \hline
% L03c    & 15 & 1  & 0  & 1  & 0.94 & 0.94 & 0.94 & 9.01          & 8.28        \\ 
% \hline
% L03b    & 15 & 1  & 0  & 1  & 0.94 & 0.94 & 0.94 & 2.22          & 10.17       \\ 
% \hline
% L03a    & 14 & 0  & 0  & 3  & 1.00 & 0.82 & 0.90 & 3.45          & 16.20       \\ 
% \hline
% L03d    & 14 & 0  & 0  & 1  & 1.00 & 0.93 & 0.97 & 10.63         & 8.26        \\ 
% \hline
% L03e    & 13 & 0  & 0  & 1  & 1.00 & 0.93 & 0.96 & 3.97          & 14.96       \\ 
% \hline
% L04c    & 14 & 0  & 0  & 2  & 1.00 & 0.88 & 0.93 & 3.30          & 8.26        \\ 
% \hline
% L04b    & 15 & 0  & 0  & 1  & 1.00 & 0.94 & 0.97 & 6.35          & 10.66       \\ 
% \hline
% L04a    & 15 & 0  & 0  & 2  & 1.00 & 0.88 & 0.94 & 6.21          & 7.98        \\ 
% \hline
% L04d    & 14 & 1  & 0  & 2  & 0.93 & 0.88 & 0.90 & 7.88          & 6.19        \\ 
% \hline
% L04e    & 10 & 1  & 0  & 5  & 0.91 & 0.67 & 0.77 & 4.09          & 10.14       \\ 
% \hline
% L07c    & 14 & 1  & 0  & 3  & 0.93 & 0.82 & 0.88 & 2.41          & 5.56        \\ 
% \hline
% L07b    & 13 & 0  & 0  & 3  & 1.00 & 0.81 & 0.90 & 6.56          & 9.01        \\ 
% \hline
% L07a    & 13 & 1  & 0  & 4  & 0.93 & 0.77 & 0.84 & 1.89          & 13.96       \\ 
% \hline
% L07d    & 14 & 0  & 0  & 2  & 1.00 & 0.88 & 0.93 & 1.73          & 5.22        \\ 
% \hline
% L07e    & 11  & 0  & 0  & 3  & 1.00 & 0.79 & 0.88 & 13.26         & 17.80       \\ 
% \hline
% L08c    & 15 & 0  & 0  & 1  & 1.00 & 0.94 & 0.97 & 2.52          & 8.74        \\ 
% \hline
% L08b    & 14 & 1  & 0  & 2  & 0.93 & 0.88 & 0.90 & 11.99         & 24.48       \\ 
% \hline
% L08a    & 15 & 0  & 0  & 2  & 1.00 & 0.88 & 0.94 & 2.38          & 8.94        \\ 
% \hline
% L08d    & 13 & 0  & 0  & 1  & 1.00 & 0.93 & 0.96 & 9.57          & 5.45        \\ 
% \hline
% L08e    & 14 & 1  & 0  & 1  & 0.93 & 0.93 & 0.93 & 8.14          & 17.82       \\ 
% \hline
% L09c    & 15 & 2  & 0  & 1  & 0.88 & 0.94 & 0.91 & 2.90          & 12.02       \\ 
% \hline
% L09b    & 15 & 1  & 0  & 1  & 0.94 & 0.94 & 0.94 & 2.26          & 13.54       \\ 
% \hline
% L09a    & 14 & 0  & 0  & 3  & 1.00 & 0.82 & 0.90 & 3.29          & 10.03       \\ 
% \hline
% L09d    & 13 & 1  & 0  & 2  & 0.93 & 0.87 & 0.90 & 2.12          & 12.03       \\ 
% \hline
% L09e    & 13 & 0  & 0  & 2  & 1.00 & 0.87 & 0.93 & 4.14          & 14.66       \\ 
% \hline
% F09d    & 21 & 0  & 0  & 2  & 1.00 & 0.91 & 0.96 & 3.44          & 8.71        \\ 
% \hline
% Average &    &    &    &    & 0.95 & 0.86 & 0.89 & 5.27          & 17.27       \\
% \hline
% \end{tabular}
% \label{Tab:results_nuestra-60}

% \end{table}


The upper row of Figure \ref{fig:analysis}
illustrates how the method performs in the presence of knots. The disk F04c fails to detect the first and third rings, identifies a false ring over the knot, and misses the last ring. Despite these errors, the method detected 19 rings, with only one false detection, and missed two rings, resulting in an F1-Score of 90\%. The lower row of \Cref{fig:analysis} shows the CS-TRD results for disk L09e. Despite two significant cracks and several fungus stains, the method successfully detects 13 out of 15 rings, with one false detection. As a result, it achieves an F1-Score of 90\%. 


\begin{figure*}[ht!]
%\begin{centering}
%\begin{subfigure}{\textwidth}
\begin{centering}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\linewidth]{figures/experiments/f04c_chains.jpg}
\caption{Chains}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\linewidth]{figures/experiments/f04c_output.jpg}
\caption{Output}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\linewidth]{figures/experiments/f04c_dt_and_gt.jpg}
\caption{Gt and Dt}
\end{subfigure}

%\label{fig:f04c_analysis}
%\end{subfigure}
%\begin{subfigure}{\textwidth}
%\begin{centering}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\linewidth]{figures/experiments/l09e_chains}
\caption{Chains}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\linewidth]{figures/experiments/l09e_output}
\caption{Output}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\linewidth]{figures/experiments/l09e_dt_and_gt}
\caption{Gt and Dt}
\end{subfigure}
%\label{fig:l09e_analysis}
%\end{centering}
%\end{subfigure}
\caption{Upper row: CS-TRD result for disk F04c. Note the impact of the knot on the edge detection step. (a) chains, (b) detected rings, (c) GT rings in green, and detected rings in red. Lower row: CS-TRD result for disk L09e. The method successfully detects almost all the rings (FN=2 and FP=0) despite cracks and fungus stains. (d) chains, (e) detected rings, (f) GT rings in green, and detected rings in red.}
\label{fig:analysis}
\end{centering}
\end{figure*}



\begin{figure*}[ht!]
\begin{centering}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/ac1_output.jpg}
    \caption{AbiesAlba1}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/ac2_output.jpg}
    \caption{AbiesAlba2}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/ac3_output.jpg}
    \caption{AbiesAlba3}
    \end{subfigure}
   \caption{CS-TRD results for images from the Kennel dataset with $1500\times1500$ image size and $\sigma=2.5$.}
   \label{fig:ddbb_ac_output}
\end{centering}
\end{figure*}



Some results for the Kennel dataset are shown in \Cref{fig:ddbb_ac_output}. The results for the whole dataset can be seen in the supplementary material. The mean F-Score is 0.97 (\Cref{tab:best_res}). At most, three rings are not detected per disk. In the worst case, one ring is mistakenly detected per image, usually the last one (which is sometimes incomplete) or the core.  In \Cref{fig:ac1_analysis}, we illustrate the example of disk \textit{AbiesAlba1}. The edge parameter is set too high ($\sigma=2.5$), causing the edge detector to fail to detect the pith. Additionally, the red chain in \Cref{fig:ac1_analysis}.c is not closed because its size is smaller than 180 degrees (the $information\_threshold$ parameter is fixed once and for all). However, the method effectively detects the rings over the knot. %\Cref{tab:resultsKennel} shows that the \textit{AbiesAlba1} disk has three false negatives. The third one is the last ring, which is not detected. Note that it detects the border, which is a false positive, as illustrated in ~\Cref{fig:ddbb_ac_output}.a.

\begin{figure*}[ht]
\begin{centering}
\begin{subfigure}{0.3\textwidth}
\begin{centering}
\includegraphics[width=\linewidth]{filter_ac1.png}
\caption{Filter}
\label{fig:ac1_filter}
\end{centering}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\begin{centering}
\includegraphics[width=\linewidth]{chains_ac1.png}
\caption{Chains}
\label{fig:ac1_chains}
\end{centering}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\begin{centering}
\includegraphics[width=\linewidth]{post_ac1.png}
\caption{Postprocessing}
\label{fig:ac1_post}
\end{centering}
\end{subfigure}

\caption{CS-TRD result for AbiesAlba1 image from the Kennel Dataset (zoom over pith center). a) Filter stage output, b) Chain stage output, c) Postprocessing stage output. In a) and b), we can see that the method fails to detect edges for the pith. The $\sigma$ threshold may be too high to detect things at this resolution. In c), we can see that the red chain was not closed due to a size smaller than the $information\_threshold$ value (180)}.

\label{fig:ac1_analysis}
\end{centering}
\end{figure*}




\subsection{Comparison between CS-TRD and INBD methods.}
\input{inbd_experiments}



==> CSTRD_IPOL_v1/implementation.tex <==
\label{sec:implementation}

The implementation was made in Python 3.11. The \textit{readme.md} file on the code repository contains all the information needed to run the code.
%\subsection{Input and Output}
The demo requires, as input, an image of a tree slice and the pith position.
%\noindent A command line execution example is:
%\begin{lstlisting}[language=bash]
%  $ python main.py --input IMAGE_PATH --cx CX --cy CY 
% --output_dir OUTPUT_DIR --root REPO_ROOT_DIR
%\end{lstlisting}
\Cref{tab:parameter} summarizes the method parameters, which the user can modify if needed. 
As output, the method returns a JSON file with the tree-rings position in Labelme format \cite{wada}. 

%The parameters of the program are the following:
%\begin{itemize}
%    \item --input: path to the segmented image.
%    \item --cx: pith x's coordinate.
%    \item --cy: pith y's coordinate.
%    \item --output\_dir: directory where intermediate and final results are saved.
%    \item --root: repository root path
%\end{itemize}


%\subsection{Parameters}
%\label{sec:parameters}

%Program command line parameters are the following:
%\begin{itemize}
%    \item --sigma: Gaussian filtering standard deviation $\sigma$.
%    \item --th\_low: Low threshold on the gradient module for the Canny Devernay filter.
%    \item --th\_high: High threshold on the gradient module for the Canny Devernay filter.
%    \item --height: Image height after the resizing process.
%    \item --width: Image width after the resizing process.
%    \item --alpha: Threshold on the collinearity of the edge filtering.% (\Cref{equ:filter}).
%    \item --nr: Total number of rays.
%    \item --min\_chain\_lenght: Minimum chain length.
%\end{itemize}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
& stage & Parameter & Description & Default    \\ \hline
Basic & Edges detector & --sigma &Gaussian filtering $\sigma$  & 3       \\ \cline{2-5} 
& Preprocessing & --height & Rezised image height         &  None\\ \cline{3-5}
& & --width & Rezised image width &  None\\ \cline{2-5}
& Filtering, sampling, connect && Pith Position  & Required\\ \hline
Advanced  & Edges detector  & --th\_low &Gradient threshold low & 5\\ \cline{3-5} 
&  & --th\_high & Gradient threshold high & 15 \\ \cline{2-5} 
& Edges filtering  &--alpha & Collinearity threshold ($\alpha$) & 30° \\ \cline{2-5} 
& Sampling  & --nr &Number of rays ($N_r$)  & 360        \\ \cline{3-5} 
&  & --min\_chain\_lenght &Minimum chain length                      & 2          \\ \hline
\end{tabular}
\caption{Method parameters. The user can modify basic parameters in the demo.}
\label{tab:parameter}
\end{table}


%\subsection{Installation and Use}
%The main program language is Python. However, the edge detector stage uses the code in C from IPOL (\cite{DevernayIPOL}) and must be compiled. The source code is included in our repository because some minor modifications were made to extract the image gradient.

%The procedure to install the application is the following:

%\begin{lstlisting}[language=bash]
%  $ cd repo_root/
%\end{lstlisting}
%\begin{lstlisting}[language=bash]
%  $ conda create --name ipol
%  $ conda activate ipol
%  $ conda install -n ipol -c conda-forge geos
%  $ conda install -n ipol -c anaconda cmake 
%  $ conda install -n ipol pip
%\end{lstlisting}
%\begin{lstlisting}[language=bash]
%  $ pip3 install --no-cache-dir -r requirements.txt
%\end{lstlisting}

%\begin{lstlisting}[language=bash]
%  $ cd ./externas/devernay_1.0 && make clean && make
%\end{lstlisting}



==> CSTRD_IPOL_v1/inbd_experiments.tex <==
\label{sec:inbd}

To our knowledge, the only other method with available code for automatically detecting tree rings in wood cross-section images is the Iterative Next Boundary Detection Instance Segmentation (INBD) proposed by Gillert et al. \cite{inbd}. Note that this method was designed for Microscopy Images of Shrub Cross Sections, which differ from the ones we are working with regarding image resolution and species characteristics. In the INBD method, the image is segmented into the background, ring boundaries, and the pith region. Then, the circular image is transformed into polar coordinates using the pith's center as the origin. Iterative image patches are then extracted, and rings are segmented individually from the inner to the outer rings. Both stages employ a U-NET network.

Furthermore, the ground truth pith location is used as input in the experiments for the CS-TRD. To ensure a fair comparison, the second stage of the INBD method is modified to take the pith boundary as input.

%To our knowledge, the only method with available code for tree ring delineation over wood cross-section images is the one proposed at \cite{inbd}. They proposed an Iterative Next Boundary Detection Instance Segmentation method (INBD) for tree ring delineation in Microscopy Images of Shrub Cross Sections. It comprises two stages: in the first stage, three classes are segmented in the image: background, ring boundaries, and the pith region. In the second stage, the disk image is transformed to polar coordinates using the mass center of the pith. Iterative image patches are extracted, where a ring is segmented individually, starting from the inner to the outer rings. Both stages use a U-NET network. Additionally, in the experiments made for the CS-TRD, the ground truth pith location is used as input. To be fair in the comparison, INBD's second stage is modified to take the pith boundary as input. 
 
%\textcolor{blue}{El unico metodo con codigo disponible para delineamiento de anillos sobre imagenes de cortes transversales es el propuesto en \cite{https://doi.org/10.48550/arxiv.2212.03022}. Este metodo es un metodo de learning completamente automatic que busca delinear los anillos. Esta compuesto de dos etapas: en la primera etapa se segmentan cuatro categorias en la imagen: el background, anillos, frontera entre anillos y el centro. En la segunda etapa, dado el centro, se segmentan los anillos pero en coordenadas polares de manera iterativa. Se toma el perimetro del centro como frontera de anillo 0. Luego en coordenadas polares, dado el anillo i (i=0) se infiere el anillo i+1 (1). Este procedimiento se realiza de manera iterativa hasta llegar el borde del disko (background). En cada iteracion se toma una seccion rectangular de la imagen que incluye al anillo i y al anillo i+1 (idealmente). En ambas etapas se utiliza la red UNET para segmentar. Por mas detalles consultar el articulo. }



%\textcolor{blue}{En los experimentos presentados por el metodo CS-TRD se utiliza el centro groud truth. Para ser justos con la comparacion, se modifica el metodo INBD para utilizar el centro verdadero en la segunda etapa. Para ser mas exactos, el metodo INBD utiliza el perimetro de la medula (anillo 0) asi como su centro de masa ( eje para convertir a polares). }

To train the INBD model with the UruDendro dataset, we randomly divided it into train, validation, and test sets with 40, 12, and 12 images, respectively. Guillert et al. trained their model with the EH dataset, which consists of 82 images with 949 rings. Our UruDendro dataset comprises 64 images and 1123 rings. For training the INBD model, each image is divided into patches determined by successive rings in polar coordinates, ensuring that each patch includes an entire ring. Even though the EH dataset has more images, the UruDendro dataset has more rings per image. Considering the total number of tree rings, both datasets are comparable.

%In order to train the INBD model with the UruDendro dataset, we randomly divided it into train, validation, and test sets with 40, 12, and 12 images, repectively. Guillert et al. train their model with the EH dataset \cite{inbd}, which has 82 images with a total of 949 rings. Our UruDendro dataset has 64 images and 1123 rings. To train the INBD model, each image is split into patches determined by successive rings in polar coordinates in such a way that each patch includes an entire ring. Therefore, considering that the EH dataset has more images but the UruDendro one has more rings per image, we conclude that both datasets are comparable in (considering the total number of tree rings). 

%\textcolor{blue}{Para entrenar y evaluar el metodo se divide de manera aleatoria el dataset en 3 subconjuntos: entrenamiento ( 40 imagenes), validacion (12 imagenes) y evaluacion (12 imagenes). El conjunto de validacion se utiliza para elegir los hiperparametros del metodo. La comparacion entre el metodo cstrd y este se realiza sobre el conjunto de evaluacion. En el articulo INBD se entrena y evalua el modelo con el dataset EH de 82 imagenes de diskos, donde se utilizan 24 para entrenamiento y 58 para la evaluacion. El dataset EH tiene en total 949 anillos. En el  dataset UruDendro, se utilizan diskos de aproximadamente 24 an;os en su mayoria, donde se tienen un total de 1223 anillos. Teniendo en cuenta que el metodo INBD utiliza patches de la imagen para entrenar, donde en cada patche se tiene una frontera de anillos, si bien, nuestro dataset tiene menor cantidad de imagenes (64 contra 82), tiene mas anillos (1123 contra 949). Por esto, creemos que los datos con los que contamos para la especie Pinus taeda para entrenar y evaluar el modelo INBD son comparables a los utilizados en \cite{https://doi.org/10.48550/arxiv.2212.03022}. }

The INBD method relies on two important hyperparameters: the number of iterations at each epoch (n) and the image size factor (downsample). We seek the best-performing INBD model by exploring a grid with $n \in \{1, 2, 3, 4\}$ and $downsample \in \{0, 2, 4\}$. The model was trained using the UruDendro training and validation sets. The model that exhibits the best performance on the validation set was chosen. For training, we utilized the ClusterUy infrastructure, as described in ClusterUy \cite{clusterUy}, equipped with an Nvidia Tesla P100 GPU with 12GB of RAM. The hyperparameters $n=3$ and $downsample=0$ yield the best performance on the validation set.


%The INBD method has two important hyperparameters: the number of iterations at each epoch ($n$) and the image size factor ($downsample$). We search for the best INBD model in a grid of size $n \in \{1,2,3,4\}$ and $downsample \in \{0, 2, 4\}$, where the model is trained with the train set and evaluated in the validation set. The model with the best performance over the validation set is selected. For training, we use the ClusterUy (\cite{clusterUy}) infrastructure, which has an Nvidia Tesla P100 GPU with 12GB RAM. The hyperparameters with the best performance over the validation set are $n=3$ and $downsample=0$. 

%\textcolor{blue}{El metodo INBD cuenta con dos hiperparametros importantes que son la densidad angular $\alpha$, que controla la resolucion angular, y el numero de iteraciones en una epoca de entrenamiento $n$. Para ambos hiperparametros, se utilizan los mismos rangos de valores utilizados en el articulo original. Además, dado que los experimentos se realizan en el ClusterUy (\cite{clusterUy}) se trabaja con las imagenes en resolucion original. Se selecciona el modelo con maximo desempen;o (deteccion de anillos) sobre el conjunto de validacion utilizando la metrica propuesta en \cite{https://doi.org/10.48550/arxiv.2212.03022}, where $\alpha=2\pi$ and $n=3$. }


\begin{table}[htbp]
\scriptsize
\centering
\caption{Comparative results between INBD and CS-TRD methods over the test set of images from the UruDendro dataset. To compare the execution times the same HW was used. $\uparrow$ ($\downarrow$) indicates higher (lower) values are better.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
%\textbf{Method} & \textbf{P $\uparrow$}  & \textbf{R $\uparrow$} & \textbf{F $\uparrow$} & \textbf{RMSE (pixels) $\downarrow$} & \textbf{\begin{tabular}[c]{@{}c@{}}Time CPU (seconds) $\downarrow$ \end{tabular}} \\ \hline
\textbf{Method} & \textbf{P $\uparrow$}  & \textbf{R $\uparrow$} & \textbf{F $\uparrow$} & \textbf{RMSE (pixels) $\downarrow$} & \textbf{Time CPU (seconds) $\downarrow$ }\\ \hline
INBD            & 0.75       & 0.84       & 0.79       & 5.7           & \textbf{7.5}                                                                  \\ \hline
CS-TRD          & \textbf{0.94 }      & \textbf{0.88 }      & \textbf{0.91}       & \textbf{3.0}           & 18                                                                     \\ \hline
\end{tabular}
\label{tab:inbd}
\end{table}


%\textcolor{blue}{ \Cref{tab:inbd} compara los metodos INBD and CS-TRD methods sobre UruDendro Test dataset ( \Cref{fig:inbd}). Dado que el metodo INBD es entrenado y evaluado en el ClusterUy (Nvidia Tesla P100 GPU 12 GB RAM) el tiempo de ejecucion no es comparable. Se recuerda que en este experimento interesa obtener el mejor desempen;o posible para el metodo INBD en cantidad en anillos detectados, por lo cual se entreno/evaluo con las imagenes en resolucion original. En cuanto a RMSE vemos que el metodo INBD es ligeramente superior al CS-TRD por 0.6px, lo cual es despreciable en este dataset. A modo de referencia, en el articulo UruDendro, se tiene un RMSE  minimo en la anotacion de los etiquetadores de 0.33px y un maximo RMSE de 2,565px (por mas informacion consultar la Table 3 del paper de Urudendro).}

Table \ref{tab:inbd} compares the performance of both methods using the test set from the UruDendro dataset. When using the same CPU hardware, we observe that the INBD  execution time is better, running at an average of 7.5 seconds compared to 18 seconds for CS-TRD. In terms of performance, CS-TRD outperforms the INBD model in precision, recall, and F-score. When considering the RMSE metric, CS-TRD  performs slightly better than INBD, with a difference of 2.7 pixels. As a point of reference, the RMSE difference between the human annotators on the UruDendro dataset is around 2.5 pixels.

%\Cref{tab:inbd} compares the performance of both methods over the test set from the UruDendro dataset. Using the same CPU HW, we can see that the execution time is similar, even if INBD is slightly better, running in a mean time of 7.5 against 18 seconds for CS-TRD. Considering the performance,  CS-TRD is more precise than the INBD model (0.94 vs. 0.75) and has a higher recall: 0.88 for the CS-TRD and 0.84 for the INBD. CS-TRD also beats the INBD method concerning the F-Score (0.91 vs. 0.79). Regarding the RMSE metric, INBD is slightly worse by 2.7 pixels. As a reference, in the UruDendro dataset, the maximum RMSE difference between human annotators is around 2.5 pixels. 

%\textcolor{blue}{Con respecto a los indicadores de precision ($\bold{P}$) and recall ($\bold{R}$) podemos decir que en recall ambos metodos tienen un desempen;o similar pero en precision el metodo CS-TRD es considerablemente mejor (0.913 contra 0.752). Esto se debe a que el metodo INBD por disen;o tiene una alta taza de falsos positivos segun describen los autores en \cite{https://doi.org/10.48550/arxiv.2212.03022}. }

%1. Figura que muestre a ambos metodos funcionando bien. F09b (F9A)
%2. Figura que muestre alta tasa de falsos positives en el centro. L02a.
%3. Arrastrando error iterativamente. F03b
%4. Falsos positivos en la corteza. L04a
%5. Mala. l02b (L2A_SIN_MC)


\Cref{fig:CSTRDvsINBD} illustrates a qualitative comparison between both methods for two disks of the UruDendro dataset. Subfigures a, c, e, and g superpose the detected rings in red and the ground truth rings in green, while subfigures b, d, f, and h depict the absolute radial error between the automatic detections and the GT disks. In the upper row, the results for disk F03b are shown. CS-TRD produced 20 True Positives, 1 False Positive, and 3 False Negatives, compared to 19 True Positives, 3 False Positives, and 4 False Negatives for INBD. The INBD method is iterative, and an error produced in a certain ring is propagated to the next rings outward, as seen in subfigure d. This significantly increases the RMSE error (9.2 for the INBD and 1.1 for the CS-TRD). The lower row of \Cref{fig:CSTRDvsINBD} illustrates the results for a disk with a high amount of fungus stains (L02b), which produces an important number of false detections (20) by the INBD method.  




\begin{figure*}[t]
\begin{subfigure}{\textwidth}
\begin{center}
   \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/cstrd_f03b_dt_and_gt}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/cstrd_f03b_heat_map_Spectral}
   \caption{}
   \end{subfigure}
   \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/inbd_f03b_dt_and_gt}
   \caption{}
   \end{subfigure}   
   \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/inbd_f03b_heat_map_Spectral}
   \caption{}
   \end{subfigure}
\end{center}
\end{subfigure}
\begin{subfigure}{\textwidth}
\begin{center}
    \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/cstrd_l02b_dt_and_gt}
  \caption{}
  \end{subfigure}   
  \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/cstrd_l02b_heat_map_Spectral}
   \caption{}
   \end{subfigure}
   \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/inbd_l02b_dt_and_gt}
  \caption{}
  \end{subfigure}   
  \begin{subfigure}{0.23\textwidth}
   \includegraphics[width=1\linewidth]{figures/inbd/method_comparison/inbd_l02b_heat_map_Spectral}
   \caption{}
   \end{subfigure}
\end{center}
\end{subfigure}
\caption{Upper row, results of CS-TRD (left) and INBD (right) methods for disk F03b of UruDendro. In (a) and (c), the ring detections are shown in red, and the GT rings in green. In (b) and (d) are shown the absolute radial error between the ring detections and the GT rings is displayed (read indicates a low error and blue indicates a high error.  A white band indicates no detection for a given ground truth ring. Lower row, results of CS-TRD (left) and INBD (right) methods for disk L02b of UruDendro. In (e) and (g), the ring detections are shown in red, and the GT rings in green. In (f) and (h), the absolute radial error between the ring detections and the GT rings is displayed (read indicates a low error, and blue indicates a high error. A white band indicates no detection for a given ground truth ring.}
   \label{fig:CSTRDvsINBD}
\end{figure*}


==> CSTRD_IPOL_v1/introduction.tex <==
\label{sec:intro}
Most of the available methods for dendrochronology (measurement and dating of tree growth rings) use images taken from cores (small cylinders crossing all the tree growth rings) instead of complete transverse cross sections. Figure \ref{fig:coreimg} illustrates that core images are rectangular sections. Using cores for the analysis presents some advantages. The rings are measured on a small portion of the trunk, which can be assumed as a sequence of bands with repetitive contrast, simplifying the image analysis.
However, this method provides limited information on annual tree growth because it results in a circular approximation based on a rectangular section. In many cases, ring growth is not uniform, leading to significant errors.
%However, this gives limited information on the annual tree growth since it ends up being a circular approximation of the tree growth (1 D) estimated by the rectangular section, but in many situations, the ring growth is not uniform, which induces considerable errors.
An application that needs the study of the whole cross-section is when studying the angular homogeneity of the ring-tree pattern trying to detect the so-called compression wood \cite{Duncker2014} for which the lack of homogeneity in the growing pattern produces differential mechanical properties. On the downside,
cross-section analysis implies the felling of the tree and includes the challenge of generating a pattern of (almost) concentric closed curves representing the tree rings. As Figure \ref{fig:ddbb} shows, several factors increase the difficulty of the task: wood knots, fungi appearing as black spots with shapes following radial directions, and cracks that can be very wide. 

%Several methods exist for automatically detecting tree rings in core images \cite{Norell-2009, Norell2007GreyWP, Zhou2012, Polek2022AutomationOT}. As the core approach is more popular, most available datasets used by machine learning-based methods for training are of that type and most machine learning-based approaches are designed for core images. 
%But those images give partial information on the tree-ring structure, which is essential for some applications. For example, when studying the angular homogeneity of the ring-tree pattern. An example is the detection of the so-called compression wood \cite{Duncker2014} for which the lack of homogeneity in the growing pattern produces differential mechanical properties.

This article presents a founded method for automatically delineating tree rings on cross-section RGB images. The approach takes advantage of the knowledge of the tree cross-section's general structure and redundant information on a radial profile for different angles around the tree's pith. %The principal contribution of this article is a new automatic method for detecting tree rings on RGB images of wood cross-sections. 
The method is evaluated over two public datasets with two different species and outperforms the other publicly available comparable method \cite{inbd} in accuracy.

\Cref{sec:antecedentes} briefly review previous work in the field. \Cref{sec:method} describes the proposed automatic cross-section tree-ring detection algorithm (CS-TRD). \Cref{sec:algorithm} presents in more detail the algorithms and \Cref{sec:implementation} discuss implementation details.
\Cref{sec:ExperimentsAndResults} briefly presents a dataset for developing and testing the proposed approach and discusses some experimental results. \Cref{sec:conclusions} concludes and propose future work. 


\begin{figure*}
\begin{center}
   \includegraphics[width=0.3\textwidth]{figures/introduction/picea_04r.png}
   \includegraphics[width=0.3\textwidth]{figures/introduction/larix_19r.png}
   \includegraphics[width=0.3\textwidth]{figures/introduction/abies_04r.png}
  % \includegraphics[angle=90,origin=l]{figures/abies_16.png}
   %\includegraphics[angle=90,origin=l]{figures/picea_13.png}
   \caption{Examples of core tree-ring images taken from a dataset with 239 images \cite{FABIJANSKA2017279}.}
   \label{fig:coreimg}
\end{center}
\end{figure*}


\begin{figure*}
\begin{centering}
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
    \includegraphics[width=\textwidth]{figures/introduction/F02a}
    \label{fig:ddbb-F02a}
%    \caption{F02a}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
    \includegraphics[width=\textwidth]{figures/introduction/F02b}
    \label{fig:ddbb-F02b}
%    \caption{F02b}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
    \includegraphics[width=\textwidth]{figures/introduction/F02c}
    \label{fig:ddbb-F02c}
%    \caption{F02c}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F02d}
    \label{fig:ddbb-F02d}
%    \caption{F02d}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F02e}
    \label{fig:ddbb-F02e}
%    \caption{F02e}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F03c}
    \label{fig:ddbb-F03c}
%    \caption{F03c}
%    \end{centering}
    \end{subfigure}
%    \hfill
     \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F07b}
    \label{fig:ddbb-F07b}
%    \caption{F07b}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/L02b}
    \label{fig:ddbb-L02b}
%    \caption{L02b}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/L03c}
    \label{fig:ddbb-L03c}
%    \caption{L03c}
%    \end{centering}
    \end{subfigure}
%    \hfill
   \caption{Some examples of images from the UruDendro dataset. Note the variability of the images and the presence of fungus (image L02b), knots (images F07b and F03c), and cracks (images F02e and L03c). The first five images are from the same tree at different heights, as the text explains in Section \ref{sec:database}. }
   \label{fig:ddbb}
\end{centering}
\end{figure*}

%---------------------------------------------------
%---------------------------------------------------




==> CSTRD_IPOL_v1/method.tex <==
In this section, we present the main ideas of the method for tree-ring delineation over RGB cross-section images, called  CS-TRD for Cross-Section Tree-Ring Detector.
\label{sec:method}
\subsection{Assumptions}
Our tree-ring detection algorithm is heavily based on the structural characteristics of the problem:
\begin{itemize}
    \item The use of the whole horizontal cross-section of a tree (slice) instead of a wood dowel (or core), as most dendrochronology approaches do. 
    \item The following properties generally define the rings on a slice:
    \begin{enumerate}
        \item The rings are roughly concentric, even if their shape is irregular. This means that two rings can't cross.
        \item Several rays can be traced outwards from the slice pith. Those rays will cross each ring only once.
        \item We are interested only in the rings corresponding to the latewood to earlywood transitions, namely the \textit{annual rings}.
        \end{enumerate}
\end{itemize}



The principal idea of the method proposed in this work is the definition and use of a general structure formed by the rings, as explained in \Cref{sec:definitions}. %This global structure is pretty general and can be used for other problems related to tree rings. For instance, the same general structure is used for the proposed automatic detection method and the design of the interactive manual delineation tool.

\subsection{Definitions}
\label{sec:definitions}
\begin{figure*}
\begin{center}
   \begin{subfigure}{0.40\textwidth}
   \def\svgwidth{\linewidth}
   \input{SpyderWebb.pdf_tex}
   \caption{}
   \label{fig:definitionsA}
   \end{subfigure}
   \hfill
   \begin{subfigure}{0.40\textwidth}
   \def\svgwidth{\linewidth}
   \input{ChainPuntosYNodosGrande_Layer_1.pdf_tex}
   \caption{}
   \label{fig:definitionsB}
   \vspace{5pt}
   \def\svgwidth{\linewidth}
   \input{dosChainsCellsYnodos_Layer_1.pdf_tex}
   \caption{}
   \hfill
   \label{fig:definitionsC}
   \end{subfigure}
   \caption{(a) The whole structure, called \textit{spider web}, is formed by a \textit{center} (which corresponds to the slice pith), $N_r$ \textit{rays} (in the drawing $N_r=18$) and the \textit{rings} (concentric curves). In the scheme, the \textit{rings} are circles, but in practice, they can be (strongly) deformed as long as they don't intersect another \textit{ring}. Each ray intersects a ring only once in a point called \textit{node}. (b) A curve is a set of connected \textit{points} (small green dots). Some of those \textit{points} are the intersection with \textit{rays}, named \textit{nodes} (black dots). A chain is a set of connected \textit{nodes}. In this case, the \textit{node} $N_i$ is the \textit{point} $p_n$. (c) Each \textit{Chain} $Ch_k$ and $Ch_{k+1}$, intersects the  \textit{rays} $r_{m-1}$, $r_{m}$ and $r_{m+1}$ in \textit{nodes} $N_{i-1}$, $N_{i}$ and $N_{i+1}$. %Those \textit{rays} and \textit{chains} (as well as the four corresponding \textit{nodes}) determines \textit{cells} $C_{l-1}$, $C_{l}$ and $C_{l+1}$.
   } 
   \label{fig:definitions}
\end{center}
\end{figure*}
 To explain the approach, we need some naming definitions; see Figure \ref{fig:definitions}. We call \textit{spider web} the global structure of the tree-rings we are searching for, which is depicted in a general way in  Figure \ref{fig:definitions}.a. It comprises a \textit{center}, associated with the slice's pith, which is the origin of a certain number of \textit{rays}. The \textit{rings} are concentric and closed curves that do not cross each other. Each \textit{ring} is formed by a \textit{curve} of connected points. Each \textit{ray} crosses a \textit{curve} only once. The \textit{rings} can be viewed as a \textit{curve} of points with \textit{nodes} in the intersection with the \textit{rays}. A \textit{chain} is a set of connected \textit{nodes}. As shown in Figure \ref{fig:definitions}.b, a \textit{curve}  is a set of chained nodes (small green dots in the figure, noted $P_i$). Depending on the position of the \textit{curve} concerning the \textit{center}, some of those \textit{points} are  \textit{nodes} (larger black dots in the figure, denoted $N_i$ hereafter). 
 %A \textit{node} can move along a \textit{ray} in a radial direction, but its movement in a tangential direction over the \textit{chain} is forbidden. In other words, \textit{nodes} can move along a \textit{ray} as if it were hoops sliding along the \textit{rays}. 
 The larger the number $Nr$ of \textit{rays}, the better the precision of the reconstruction of the \textit{rings}. We fix $Nr = 360$. Note that this is the ideal setting. In actual images,  \textit{rings} can disappear without forming a closed curve,  %\textit{cells} can have very varied shapes, 
 the \textit{rings} can be strongly deformed, etc. 
 
 Figure \ref{fig:definitions}.c illustrates the nomenclature used in this paper: \textit{Chains} $Ch_k$ and $Ch_{k+1}$, intersect the  \textit{rays} $r_{m-1}$, $r_{m}$ and $r_{m+1}$ in \textit{nodes} $N_{i-1}$, $N_{i}$ and $N_{i+1}$. To explain the method, we use this terminology. \textit{Chains} merge to form a \textit{ring}. The \textit{rays} determine a sampling of the \textit{curves}, producing \textit{chains}. 



\subsection{Approach}

The method takes as input an image of the disk without background and the biological center of the disk (pith) (see~\Cref{fig:algo}.b) and returns the annual rings (see~\Cref{fig:algo}.i).~\Cref{fig:algo} illustrates the output of each stage of the method, which are fully described in~\Cref{sec:algorithm}.

Briefly, the method works as follows: from the center (disk pith), rays are traced (see~\Cref{fig:definitions}.a). The Canny edge detection method is then applied to the image (see~\Cref{fig:algo}.d), and by calculating the angle between the edge normals and the rays, most of the edges that do not belong to the latewood to earlywood transitions are eliminated. At the end of this filtering stage, we obtain both noisy edges and the edges of the rings we are looking for; additionally, some edges may be missing because they were not detected (see~\Cref{fig:algo}.e). Until now, the method is similar to the one proposed by Cerda et al. \cite{CerdaHM07}; the more challenging step is how the pixels belonging to the edges are grouped to form rings. 

In the next stage, the edges obtained in the previous phase enforce the \textit{spider web} structure, which describes the general properties of the annual rings. To achieve this, all edges are subsampled using the rays of \textit{spider web}: for each edge, we only retain the intersections between it and the respective rays (the nodes), forming what we call chains (see ~\Cref{fig:algo}.f). %The elements of the chains (intersections between edges and rays) are referred to as nodes. 
The final stage involves grouping all chains that belong to the same ring by imposing the SpiderWeb structure through a smoothness condition (see ~\Cref{fig:algo}.g, ~\Cref{fig:algo}.h and~\Cref{equ:similiraty_criterio}). The chain grouping is performed iteratively to connect chains near areas with stronger edge information. Once no more chains are connected in the current neighborhood, the method moves on to the next region with strong edge information. This iterative process, which prioritizes edge information along with the smoothness condition, is the main contribution of our method to the community. Now, we describe %The next section describes 
the method in detail.

==> introduction.tex <==
\label{sec:intro}
Most of the available methods for dendrochronology (measurement and dating of tree growth rings) use images taken from cores (small cylinders crossing all the tree growth rings) instead of complete transverse cross sections. Figure \ref{fig:coreimg} illustrates that core images are rectangular sections. Using cores for the analysis presents some advantages. The rings are measured on a small portion of the trunk, which can be assumed as a sequence of bands with repetitive contrast, simplifying the image analysis.
However, this method provides limited information on annual tree growth because it results in a circular approximation based on a rectangular section. In many cases, ring growth is not uniform, leading to significant errors.
%However, this gives limited information on the annual tree growth since it ends up being a circular approximation of the tree growth (1 D) estimated by the rectangular section, but in many situations, the ring growth is not uniform, which induces considerable errors.
An application that needs the study of the whole cross-section is when studying the angular homogeneity of the ring-tree pattern trying to detect the so-called compression wood \cite{Duncker2014} for which the lack of homogeneity in the growing pattern produces differential mechanical properties. On the downside,
cross-section analysis implies the felling of the tree and includes the challenge of generating a pattern of (almost) concentric closed curves representing the tree rings. As Figure \ref{fig:ddbb} shows, several factors increase the difficulty of the task: wood knots, fungi appearing as black spots with shapes following radial directions, and cracks that can be very wide. 

%Several methods exist for automatically detecting tree rings in core images \cite{Norell-2009, Norell2007GreyWP, Zhou2012, Polek2022AutomationOT}. As the core approach is more popular, most available datasets used by machine learning-based methods for training are of that type and most machine learning-based approaches are designed for core images. 
%But those images give partial information on the tree-ring structure, which is essential for some applications. For example, when studying the angular homogeneity of the ring-tree pattern. An example is the detection of the so-called compression wood \cite{Duncker2014} for which the lack of homogeneity in the growing pattern produces differential mechanical properties.

This article presents a founded method for automatically delineating tree rings on cross-section RGB images. The approach takes advantage of the knowledge of the tree cross-section's general structure and redundant information on a radial profile for different angles around the tree's pith. %The principal contribution of this article is a new automatic method for detecting tree rings on RGB images of wood cross-sections. 
The method is evaluated over two public datasets with two different species and outperforms the other publicly available comparable method \cite{inbd} in accuracy.

\Cref{sec:antecedentes} briefly review previous work in the field. \Cref{sec:method} describes the proposed automatic cross-section tree-ring detection algorithm (CS-TRD). \Cref{sec:algorithm} presents in more detail the algorithms and \Cref{sec:implementation} discuss implementation details.
\Cref{sec:ExperimentsAndResults} briefly presents a dataset for developing and testing the proposed approach and discusses some experimental results. \Cref{sec:conclusions} concludes and propose future work. 


\begin{figure*}
\begin{center}
   \includegraphics[width=0.3\textwidth]{figures/introduction/picea_04r.png}
   \includegraphics[width=0.3\textwidth]{figures/introduction/larix_19r.png}
   \includegraphics[width=0.3\textwidth]{figures/introduction/abies_04r.png}
  % \includegraphics[angle=90,origin=l]{figures/abies_16.png}
   %\includegraphics[angle=90,origin=l]{figures/picea_13.png}
   \caption{Examples of core tree-ring images taken from a dataset with 239 images \cite{FABIJANSKA2017279}.}
   \label{fig:coreimg}
\end{center}
\end{figure*}


\begin{figure*}
\begin{centering}
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
    \includegraphics[width=\textwidth]{figures/introduction/F02a}
    \label{fig:ddbb-F02a}
%    \caption{F02a}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
    \includegraphics[width=\textwidth]{figures/introduction/F02b}
    \label{fig:ddbb-F02b}
%    \caption{F02b}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
    \includegraphics[width=\textwidth]{figures/introduction/F02c}
    \label{fig:ddbb-F02c}
%    \caption{F02c}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F02d}
    \label{fig:ddbb-F02d}
%    \caption{F02d}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F02e}
    \label{fig:ddbb-F02e}
%    \caption{F02e}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F03c}
    \label{fig:ddbb-F03c}
%    \caption{F03c}
%    \end{centering}
    \end{subfigure}
%    \hfill
     \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/F07b}
    \label{fig:ddbb-F07b}
%    \caption{F07b}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/L02b}
    \label{fig:ddbb-L02b}
%    \caption{L02b}
%    \end{centering}
    \end{subfigure}
%    \hfill
    \begin{subfigure}{0.3\textwidth}
%    \begin{centering}
   \includegraphics[width=\textwidth]{figures/introduction/L03c}
    \label{fig:ddbb-L03c}
%    \caption{L03c}
%    \end{centering}
    \end{subfigure}
%    \hfill
   \caption{Some examples of images from the UruDendro dataset. Note the variability of the images and the presence of fungus (image L02b), knots (images F07b and F03c), and cracks (images F02e and L03c). The first five images are from the same tree at different heights, as the text explains in Section \ref{sec:database}. }
   \label{fig:ddbb}
\end{centering}
\end{figure*}

%---------------------------------------------------
%---------------------------------------------------



